ErrorCompensatedX: error compensation for variance reduced algorithms

Communication cost is one major bottleneck for the scalability for distributed learning. One approach to reduce the communication cost is to compress the gradient during communication. However, directly compressing the gradient decelerates the convergence speed, and the resulting algorithm may diverge for biased compression. Recent work addressed this problem for stochastic gradient descent by adding back the compression error from the previous step. This idea was further extended to one class of variance reduced algorithms, where the variance of the stochastic gradient is reduced by taking a moving average over all history gradients. However, our analysis shows that just adding the previous step's compression error, as done in existing work, does not fully compensate the compression error. So, we propose ErrorCompensatedX, which uses the compression error from the previous two steps. We show that ErrorCompensatedX can achieve the same asymptotic convergence rate with the training without compression. Moreover, we provide a unified theoretical analysis framework for this class of variance reduced algorithms, with or without error compensation.

==> strongly.tex <==
\onecolumn
{\huge Supplementary}

In the supplementary, we first prove the updating rule of \CR. Then we will present the detailed proof for Theorem~\ref{theo:general_nonconvex} followed by the detailed convergence rate result for each algorithm.
\section{Updating rule of \CR}
The updating rule of Algorithm~\ref{alg1} admits the form
\begin{align*}
\oe_t = & (1-\beta)\oe_{t-1} + \beta\left(\frac{\alpha_{t-1}}{\alpha_t}(2-\alpha_t)\odelta_{t-1} + \frac{\alpha_{t-2}}{\alpha_t} (1-\alpha_t)\odelta_{t-2}  \right)\\
\v_t =&  (1-\alpha_t)\v_{t-1} + \alpha_t\ob_t(\x_t) -\alpha_t\odelta_t +  \alpha_t\oe_t,\\
\x_{t+1} =& \x_t - \gamma\v_t. 
\end{align*}
where
\begin{align*}
\nonumber
\oe_t := & \frac{1}{n}\sum_{i}\e_t^\bi + \e_t,\\
\odelta_t := & \bm{\delta}_t + \frac{1}{n} \sum_{i=1}^n \bm{\delta}_{t}^{(i)},\\
\ob_t(\x): = & \frac{1}{n}\sum_i \mathscr{A}\left(\x_t;\xi_t^{(i)}\right).
\end{align*}
\begin{proof}
From the algorithm description in Algorithm~\ref{alg1}, we shall see that we are essentially using $\v_t$ as the gradient estimator of the full gradient. From the updating rule of $\v_t$, we have
\begin{align*}
\v_t
=& (1-\alpha_t)\v_{t-1} +\alpha_t C_{\omega}\left[\Delta_t\right]\\
= & (1-\alpha_t)\v_{t-1} + \alpha_t\left( \Delta_t - \bdelta_t\right)\\
 = & (1-\alpha_t)\v_{t-1} + \frac{\alpha_t}{n}\sum_{i}C_{\omega}\left[ \Delta_t^{(i)}  \right]+ \alpha_t\e_t - \alpha_t \bdelta_t\\
= & (1-\alpha_t)\v_{t-1} + \frac{\alpha_t}{n}\sum_{i}\left( \Delta_t^{\bi} - \bdelta_{t}^{(i)} \right) + \alpha_t\e_t - \alpha_t \bdelta_t\\
= & (1-\alpha_t)\v_{t-1}+ \frac{\alpha_t}{n}\sum_{i}\left(  \mathscr{A}\left(\x_t;\xi_t^{(i)}\right)  + \e_t^\bi - \bdelta_{t}^{(i)} \right)+ \alpha_t\e_t - \alpha_t \bdelta_t\\
= & (1-\alpha)\v_{t-1} + \alpha_t\ob_t(\x_t) + \alpha_t\oe_t - \alpha_t\odelta_t.
\end{align*}
Notice that in the deduction above we continuously using the fact that $C_{\omega}[\x] = \x - \bdelta$.
For $\oe_t$, we have
\begin{align*}
\oe_t =& \frac{1}{n}\sum_{i}\e_t^\bi + \e_t\\
= & \frac{1-\beta}{n}\sum_{i}\e_{t-1}^\bi + \frac{\beta}{n}\sum_{i}\left(\frac{\alpha_{t-1}}{\alpha_t}(2-\alpha_t)\delta_{t-1}^\bi + \frac{\alpha_{t-2}}{\alpha_t} (1-\alpha_t)\delta_{t-2}^\bi  \right)\\
&+ (1-\beta)\e_{t-1} + \beta\left(\frac{\alpha_{t-1}}{\alpha_t}(2-\alpha_t)\delta_{t-1} + \frac{\alpha_{t-2}}{\alpha_t} (1-\alpha_t)\delta_{t-2}  \right)\\
= & (1-\beta)\oe_{t-1} + \beta\left(\frac{\alpha_{t-1}}{\alpha_t}(2-\alpha_t)\odelta_{t-1} + \frac{\alpha_{t-2}}{\alpha_t} (1-\alpha_t)\odelta_{t-2}  \right),
\end{align*}
which completes the proof.
\end{proof}

\subsection{Proof to Lemma~\ref{lemma:intuition}}\label{proof:lemma1}
\begin{proof}
For \textbf{uncompressed training}, we have
\begin{align*}
\v_t^{\text{full}} =& (1-\alpha)\v_{t-1}^{\text{full}} + \alpha\b_t\\
= & (1-\alpha)^t \v_0^{\text{full}} + \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s\\
= & \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s.
\end{align*}
Therefore the final model gets
\begin{align*}
\x_T^{\text{full}} = \x_1^{\text{full}} - \gamma\sum_{t=1}^T\v_t = \x_1^{\text{full}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s.\numberthis\label{lemma1:full}
\end{align*}
For compressed training \textbf{without compensation}, we get 
\begin{align*}
\v_t^{\text{zero}} = & (1-\alpha)\v_{t-1}^{\text{zero}} + \alpha\b_t - \bdelta_t\\
= & (1-\alpha)^t \v_0^{\text{zero}} + \sum_{s=1}^t(1-\alpha)^{t-s}(\alpha\b_s - \bdelta_s).
\end{align*}
Therefore the final model becomes
\begin{align*}
\x_T^{\text{zero}} = \x_1^{\text{zero}} - \gamma\sum_{t=1}^T\v_t = \x_1^{\text{zero}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s - \gamma\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}  \bdelta_s.
\end{align*}
Notice that  we have
\begin{align*}
\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\bdelta_{s} = & \sum_{s=1}^{T}\sum_{t=s}^T(1-\alpha)^{t-s}\bdelta_{s}\\
= & \frac{1}{\alpha}\sum_{s=1}^{T}\left( 1 - (1-\alpha)^{T-s+1} \right)\bdelta_s,\numberthis\label{lemma1:eq2}
\end{align*}
which leads to 
\begin{align*}
\x_T^{\text{zero}} =&\x_1^{\text{zero}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s - \frac{\gamma}{\alpha}\sum_{s=1}^{T}\left( 1 - (1-\alpha)^{T-s+1} \right)\bdelta_s\\
= & \x_T^{\text{full}} - \frac{\gamma}{\alpha}\sum_{s=1}^{T}\left( 1 - (1-\alpha)^{T-s+1} \right)\bdelta_s.
\end{align*}
For \textbf{single compensation}, the gradient estimator is updated following
\begin{align*}
\v_t^{\text{one}} = &(1-\alpha)\v_{t-1}^{\text{one}} + \alpha\b_t + \bdelta_{t-1}  - \bdelta_t\\
= & (1-\alpha)^t \v_0^{\text{one}} + \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s + \sum_{s=1}^t(1-\alpha)^{t-s}(\bdelta_{s-1}  - \bdelta_s)\\
= & \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s + \sum_{s=1}^t(1-\alpha)^{t-s}(\bdelta_{s-1}  - \bdelta_s).
\end{align*}
Then the final model becomes
\begin{align*}
\x_T^{\text{one}} = \x_1^{\text{one}} - \gamma\sum_{t=1}^T\v_t = \x_1^{\text{one}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s + \gamma\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}(\bdelta_{s-1}  - \bdelta_s).\numberthis\label{lemma1:eq1}
\end{align*}
For $\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\bdelta_{s-1}$ we have
\begin{align*}
\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\bdelta_{s-1} = & \frac{1}{1-\alpha}\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-(s-1)}\bdelta_{s-1}\\
=& \frac{1}{1-\alpha}\sum_{t=1}^T\sum_{s=0}^{t-1}(1-\alpha)^{t-s}\bdelta_{s}\\
=& \frac{1}{1-\alpha}\sum_{s=0}^{T-1}\sum_{t=s+1}^T(1-\alpha)^{t-s}\bdelta_s\\
= & \frac{1}{\alpha}\sum_{s=1}^{T-1}\left( 1 - (1-\alpha)^{T-s} \right)\bdelta_s.\numberthis\label{lemma1:eq3}
\end{align*}
Then taking \eqref{lemma1:eq2} and \eqref{lemma1:eq3} into \eqref{lemma1:eq1} we get
\begin{align*}
\x_T^{\text{one}} = & \x_1^{\text{one}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s  - \gamma\bdelta_T +\frac{\gamma}{\alpha} \sum_{s=1}^{T-1}\left((1-\alpha)^{T-s+1} - (1-\alpha)^{T-s}\right)\bdelta_s\\
= & \x_1^{\text{one}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s  - \gamma\bdelta_T  - \gamma\sum_{s=1}^{T-1}(1-\alpha)^{T-s}\bdelta_s\\
= & \x_T^{\text{full}} - \gamma\bdelta_T - \gamma \sum_{s=0}^{T-1}(1-\alpha)^{T-s}\bdelta_s.
\end{align*}
For {\CR}, we have
\begin{align*}
\v_t^{\text{two}} =& (1-\alpha)\v_{t-1}^{\text{two}} + \alpha\b_t + (2-\alpha)\bdelta_{t-1} - (1-\alpha)\bdelta_{t-2} - \bdelta_t,
\end{align*}
which leads to
\begin{align*}
\v_t^{\text{two}} + \bdelta_t - \bdelta_{t-1} =& (1-\alpha)(\v_{t-1}^{\text{two}} + \bdelta_{t-1} - \bdelta_{t-2}) + \alpha\b_t \\
= & (1-\alpha)^t (\v_0^{\text{two}} + \bdelta_0 - \bdelta_{-1}) + \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s\\
= & \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s,
\end{align*}
which means
\begin{align*}
\v_t^{\text{two}} = \alpha\sum_{s=1}^t(1-\alpha)^{t-s}\b_s -\bdelta_t + \bdelta_{t-1}.
\end{align*}
In this case, the final model gets
\begin{align*}
\x_T^{\text{two}} =& \x_1^{\text{two}} - \gamma\sum_{t=1}^T\v_t\\
=& \x_1^{\text{two}} - \gamma\alpha\sum_{t=1}^T\sum_{s=1}^t(1-\alpha)^{t-s}\b_s - \bdelta_T\\
= &\x_T^{\text{full}} - \gamma  \bdelta_T.
\end{align*}
\end{proof}







% \newpage
% \begin{lemma}\label{lemma:bound_delta}
% For {\CR}, under Assumptions xx, defining
% \begin{align*}
% D_\omega = \frac{480\omega^2}{(1-15\omega^2)(1-12\omega^2)},
% \end{align*} then the compression error can be upper bounded by
% \begin{align*}
% \sum_{t=0}^{T-1}\mathbb{E}\|\odelta_t\|^2
% \leq D_{\omega}L^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\left\|\u_{t-1} \right\|^2 + 2D_{\omega}\alpha^2\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + 2D_{\omega}\alpha^2(\sigma^2 + \zeta^2)T,
% \end{align*}
% if we have
% \begin{align*}
% 1-15\omega^2 > & 0,\\
% (3\alpha^2 + L^2\gamma^2)\leq &  \frac{1}{2D_\omega}.
% \end{align*}
% \end{lemma}

% \begin{proof}
% From the definition of $\Delta_t^\bi$ we get
% \begin{align*}
%  &   \mathbb{E}\|\Delta_t^\bi\|^2\\
% = &  \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\v_{t-1} - (1-\alpha)\g_t^\bi(\x_{t-1})+ (2-\alpha) \bm{\delta}^{(i)}_{t-1} - (1-\alpha)\bdelta_{t-2}^{(i)} \right\|^2\\
% = &  \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\left(\u_{t-1} - \odelta_{t-1} + \odelta_{t-2} \right) - (1-\alpha)\g_t^\bi(\x_{t-1})+ (2-\alpha) \bm{\delta}^{(i)}_{t-1} - (1-\alpha)\bdelta_{t-2}^{(i)} \right\|^2\\
% = &  \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\u_{t-1} - (1-\alpha)\g_t^\bi(\x_{t-1})+ (2-\alpha) \bm{\delta}^{(i)}_{t-1} - (1-\alpha)\bdelta_{t-2}^{(i)} + \alpha(\odelta_{t-1} - \odelta_{t-2}) \right\|^2\\
% \leq & (1+2) \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\u_{t-1} - (1-\alpha)\g_t^\bi(\x_{t-1})\right\|^2+ \left(1+\frac{1}{2}\right)  \mathbb{E} \left\|(2-\alpha) \bm{\delta}^{(i)}_{t-1} - (1-\alpha)\bdelta_{t-2}^{(i)} + \alpha(\odelta_{t-1} - \odelta_{t-2}) \right\|^2\\
% \leq & 3 \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\u_{t-1} - (1-\alpha)\g_t^\bi(\x_{t-1})\right\|^2+ \frac{3}{2}\left( \frac{10}{9}\mathbb{E} \left\|(2-\alpha) \bm{\delta}^{(i)}_{t-1} - (1-\alpha)\bdelta_{t-2}^{(i)}\right\|^2 + 10\mathbb{E}\left\| \alpha(\odelta_{t-1} - \odelta_{t-2}) \right\|^2  \right)\\
% \leq & 3 \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\u_{t-1} - (1-\alpha)\g_t^\bi(\x_{t-1})\right\|^2+ \left( 10\mathbb{E} \left\| \bm{\delta}^{(i)}_{t-1}\right\|^2 +5 \left\|\bdelta_{t-2}^{(i)}\right\|^2 + 15\mathbb{E}\left\| \alpha(\odelta_{t-1} - \odelta_{t-2}) \right\|^2  \right)\\
% \leq & 3 \mathbb{E}\left\|\g_t^\bi(\x_t) - \alpha\u_{t-1} - (1-\alpha)\g_t^\bi(\x_{t-1})\right\|^2+   \left(10\mathbb{E} \left\|\bm{\delta}^{(i)}_{t-1}\right\|^2 + 15\mathbb{E}\left\| \bdelta_{t-2}^{(i)} \right\|^2  + 30\alpha^2\mathbb{E} \left\|\odelta_{t-1}\right\|^2 + 30\alpha^2\mathbb{E}\left\| \odelta_{t-2}^{(i)} \right\|^2 \right)\\
% \leq & 3 \mathbb{E}\left\|\left(\g_t^\bi(\x_t)-\g_t^\bi(\x_{t-1}) \right) - \alpha\left(\u_{t-1} - \g_t^\bi(\x_{t-1}) \right)\right\|^2+ \left(10\mathbb{E} \left\|\bm{\delta}^{(i)}_{t-1}\right\|^2 +5 \mathbb{E}\left\| \bdelta_{t-2}^{(i)} \right\|^2\right) + 30\alpha^2\left(\mathbb{E} \left\|\odelta_{t-1}\right\|^2 + \mathbb{E}\left\| \odelta_{t-2}^{(i)} \right\|^2\right)\\
% \leq & 6\mathbb{E}\left\|\g_t^\bi(\x_t)-\g_t^\bi(\x_{t-1}) \right\|^2 + 6 \alpha^2\mathbb{E}\left\| \u_{t-1} - \g_t^\bi(\x_{t-1}) \right\|^2+ 10\mathbb{E} \left\|\bm{\delta}^{(i)}_{t-1}\right\|^2 + 5\mathbb{E}\left\| \bdelta_{t-2}^{(i)} \right\|^2\\
% &+ 30\alpha^2\left(\mathbb{E} \left\|\odelta_{t-1}\right\|^2 + \mathbb{E}\left\| \odelta_{t-2}^{(i)} \right\|^2\right)\\
% \leq & 6L^2\gamma^2\mathbb{E}\left\|\v_{t-1} \right\|^2 + 6 \alpha^2\mathbb{E}\left\| \u_{t-1} - \g_t^\bi(\x_{t-1}) \right\|^2+ 10 \mathbb{E} \left\|\bm{\delta}^{(i)}_{t-1}\right\|^2 + 5\mathbb{E}\left\| \bdelta_{t-2}^{(i)} \right\|^2 + 30\alpha^2\left(\mathbb{E} \left\|\odelta_{t-1}\right\|^2 + \mathbb{E}\left\| \odelta_{t-2}^{(i)} \right\|^2\right).\numberthis\label{bound_delta_i:1}
% \end{align*}
% Notice that we cannot guarantee that $\mathbb{E} \g_t^\bi(\x) = \nabla f(\x)$, therefore we can only upper bound $\mathbb{E}\left\| \u_{t-1} - \g_t^\bi(\x_{t-1}) \right\|^2$ using
% \begin{align*}
% \mathbb{E}\left\| \u_{t-1} - \g_t^\bi(\x_{t-1}) \right\|^2 = & \mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1}) +\nabla f(\x_{t-1}) - \nabla f_i(\x_{t-1}) + \nabla f_i(\x_{t-1}) - \g_t^\bi(\x_{t-1}) \right\|^2\\
% \leq & 3 \mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2 +3\mathbb{E}\left\| \nabla f(\x_{t-1}) - \nabla f_i(\x_{t-1})\right\|^2 +3\mathbb{E}\left\| \nabla f_i(\x_{t-1})- \g_t^\bi(\x_{t-1}) \right\|^2\\
% \leq & 3 \mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2 +3\zeta^2 +3\sigma^2.
% \end{align*}
% Then \eqref{bound_delta_i:1} becomes
% \begin{align*}
% &\mathbb{E}\|\Delta_t^\bi\|^2\\
% \leq & 6 L^2\gamma^2\mathbb{E}\left\|\v_{t-1} \right\|^2 + 6 \alpha^2\mathbb{E}\left\| \u_{t-1} - \g_t^\bi(\x_{t-1}) \right\|^2+ 10\mathbb{E} \left\|\bm{\delta}^{(i)}_{t-1}\right\|^2 + 5\mathbb{E}\left\| \bdelta_{t-2}^{(i)} \right\|^2 + 30\alpha^2\left(\mathbb{E} \left\|\odelta_{t-1}\right\|^2 + \mathbb{E}\left\| \odelta_{t-2}^{(i)} \right\|^2\right)\\
% \leq & 6 L^2\gamma^2\mathbb{E}\left\|\v_{t-1} \right\|^2 + 18 \alpha^2\mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2 +18 \alpha^2(\sigma^2 + \zeta^2)\\
% &+10\mathbb{E} \left\|\bm{\delta}^{(i)}_{t-1}\right\|^2 + 5\mathbb{E}\left\| \bdelta_{t-2}^{(i)} \right\|^2 + 30\alpha^2\left(\mathbb{E} \left\|\odelta_{t-1}\right\|^2 + \mathbb{E}\left\| \odelta_{t-2}^{(i)} \right\|^2\right).\numberthis\label{bound_delta_i:2}
% \end{align*}
% Summing up the inequality above from $t=0$ to $t=T-1$, using the fact that $\bdelta_{-1} = \bdelta_{t-2} = \bm{0}$. We have $\sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_t^\bi\|^2 \geq \sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_{t-1}^\bi\|^2 \geq \sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_{t-2}^\bi\|^2$, then \eqref{bound_delta_i:2} becomes
% \begin{align*}
% \sum_{t=0}^{T-1}\mathbb{E}\|\Delta_t^\bi\|^2
% \leq & 6 L^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + 18 \alpha^2\sum_{t=0}^{T-1}\mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2  + 18 \alpha^2(\sigma^2 + \zeta^2)T\\
% &+ 15  \sum_{t=0}^{T-1}\mathbb{E} \left\|\bm{\delta}^{(i)}_{t}\right\|^2 + 60\alpha^2\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2\\
% \leq &6 L^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + 18 \alpha^2\sum_{t=0}^{T-1}\mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2  + 18 \alpha^2(\sigma^2 + \zeta^2)T\\
% &+ 15\omega^2  \sum_{t=0}^{T-1}\mathbb{E} \left\|\Delta^{(i)}_{t}\right\|^2 + 60\alpha^2\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2\\.\numberthis\label{bound_Delta_i}
% \end{align*}
% % This gives us
% % \begin{align*}
% % \sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_t^\bi\|^2
% % \leq &\omega^2\sum_{t=0}^{T-1}\mathbb{E}\|\Delta_t^\bi\|^2\\
% % \leq & 6 \omega^2L^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + 18\omega^2 \alpha^2\sum_{t=0}^{T-1}\mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2  + 18 \omega^2\alpha^2(\sigma^2 + \zeta^2)T\\
% % &+ 6 \omega^2 \sum_{t=0}^{T-1}\mathbb{E} \left\|\bm{\delta}^{(i)}_{t}\right\|^2 + 60\alpha^2\omega^2\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2,
% % \end{align*}
% which means if $1-15\omega^2 > 0$, then we have
% \begin{align*}
% &\sum_{t=0}^{T-1}\mathbb{E}\|\Delta_t^\bi\|^2\\
% \leq & \frac{6L^2\gamma^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + \frac{18\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\| \u_{t-1} - \nabla f(\x_{t-1})\right\|^2  + \frac{ 18\alpha^2(\sigma^2 + \zeta^2)T}{1-15\omega^2} + \frac{60\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2\\
% \leq & \frac{6L^2\gamma^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + \frac{18\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{ 18\alpha^2(\sigma^2 + \zeta^2)T}{1-15\omega^2} + \frac{60\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2.
% \end{align*}
% % Taking the sum of $\mathbb{E}\|\bdelta_t^\bi\|^2$ over all workers, this leads to
% % \begin{align*}
% % &\sum_{t=0}^{T-1}\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n\bdelta_t^\bi  \right\|^2\\
% % \leq & \frac{1}{n}\sum_{t=0}^{T-1}\sum_{i=1}^n\mathbb{E}\left\|\bdelta_t^\bi  \right\|^2\\
% % \leq & \frac{6\omega^2L^2\gamma^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + \frac{18\omega^2\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{ 18\omega^2\alpha^2(\sigma^2 + \zeta^2)T}{1-15\omega^2} + \frac{60\alpha^2\omega^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2.\numberthis\label{bound_sum_Delta_i}
% % \end{align*}

% For $\bdelta_t$, likewise, we get
% \begin{align*}
% \mathbb{E}\|\bdelta_t\|^2
% \leq &  \omega^2\mathbb{E}\|\Delta_t\|^2\\
% = & \omega^2\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n C_{\omega}\left[\Delta_t^{(i)}\right] + (2-\alpha) \bm{\delta}_{t-1} - (1-\alpha)\bdelta_{t-2}\right\|^2\\
% \leq & (1+3)\omega^2\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n C_{\omega}\left[\Delta_t^{(i)}\right]\right\|^2 +\left(1+ \frac{1}{3}\right)\omega^2\left(6\mathbb{E}\left\| \bm{\delta}_{t-1}\right\|^2 +3 \mathbb{E} \left\|\bdelta_{t-2}\right\|^2\right)\\
% \leq & \frac{4}{n}\sum_{i=1}^n\omega^2\mathbb{E}\left\| C_{\omega}\left[\Delta_t^{(i)}\right]\right\|^2 +\left(1+ \frac{1}{3}\right)\omega^2\left(6\mathbb{E}\left\| \bm{\delta}_{t-1}\right\|^2 +3 \mathbb{E} \left\|\bdelta_{t-2}\right\|^2\right)\\
% \leq & \frac{8(1+\omega^2)\omega^2}{n}\sum_{i=1}^n\mathbb{E}\left\| \Delta_t^{(i)}\right\|^2 +\left(1+ \frac{1}{3}\right)\omega^2\left(6\mathbb{E}\left\| \bm{\delta}_{t-1}\right\|^2 +3\mathbb{E} \left\|\bdelta_{t-2}\right\|^2\right),
% \end{align*}
% where in the last inequality,  we use the fact that
% \begin{align*}
% \mathbb{E}\left\| C_{\omega}\left[\Delta_t^{(i)}\right]\right\|^2 \leq & 2 \mathbb{E}\left\| C_{\omega}\left[\Delta_t^{(i)}\right] - \Delta_t^{(i)}\right\|^2 + 2\mathbb{E}\left\| \Delta_t^{(i)}\right\|^2\\
% \leq & (2 + 2\omega^2)\mathbb{E}\left\| \Delta_t^{(i)}\right\|^2.
% \end{align*}
% Summing up the inequality above from $t=0$ to $t=T-1$, we get
% \begin{align*}
% \sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_t\|^2\leq & \frac{9\omega^2}{n}\sum_{t=0}^{T-1}\sum_{i=1}^n\mathbb{E}\left\| \Delta_t^{(i)}\right\|^2 +12\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\| \bm{\delta}_{t}\right\|^2,
% \end{align*}
% which means
% \begin{align*}
% \sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_t\|^2\leq & \frac{9\omega^2}{n(1-12\omega^2)}\sum_{t=0}^{T-1}\sum_{i=1}^n\mathbb{E}\left\| \Delta_t^{(i)}\right\|^2.\numberthis\label{bound_sum_delta}
% \end{align*}

% Now we are ready to upper bound $\mathbb{E}\|\odelta_t\|^2$ finally:
% \begin{align*}
% \sum_{t=0}^{T-1}\mathbb{E}\|\odelta_t\|^2
% = & \sum_{t=0}^{T-1}\mathbb{E}\left\|\bdelta_t + \frac{1}{n}\sum_{i=1}^n \bdelta_t^{\bi}\right\|^2\\
% \leq & 10\sum_{t=0}^{T-1}\mathbb{E}\left\|\bdelta_t\right\|^2 + \frac{10}{9}\sum_{t=0}^{T-1}\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^{\bi}\right\|^2\\
% \leq & 10\sum_{t=0}^{T-1}\mathbb{E}\left\|\bdelta_t\right\|^2 + \frac{10\omega^2}{9n}\sum_{t=0}^{T-1}\sum_{i=1}^n\mathbb{E}\left\| \Delta_t^{\bi}\right\|^2\\
% \leq & \frac{\omega^2\left(10 + \frac{10}{1-12\omega^2}\right)}{n}\sum_{t=0}^{T-1}\sum_{i=1}^n\mathbb{E}\left\| \Delta_t^{\bi}\right\|^2\quad\text{(due to \eqref{bound_sum_delta})}\\
% \leq & \frac{20\omega^2}{n(1-12\omega^2)}\sum_{t=0}^{T-1}\sum_{i=1}^n\mathbb{E}\left\| \Delta_t^{\bi}\right\|^2.
% \end{align*}
% Then by applying \eqref{bound_Delta_i} to upper bound $\mathbb{E}\left\| \Delta_t^{\bi}\right\|^2$, we get
% \begin{align*}
% &\sum_{t=0}^{T-1}\mathbb{E}\|\odelta_t\|^2\\
% \leq & \frac{120\omega^2L^2\gamma^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + \frac{360\omega^2\alpha^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{360\omega^2\alpha^2(\sigma^2 + \zeta^2)T}{(1-15\omega^2)(1-12\omega^2)}\\
% &+ \frac{1200\omega^2\alpha^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2,
% \end{align*}
% here there is still one step left. We need to expand $\v_t$ as $(\u_t - \odelta_t - \odelta_{t-1})$, and this leads to
% \begin{align*}
% &\sum_{t=0}^{T-1}\mathbb{E}\|\odelta_t\|^2\\
% \leq & \frac{240\omega^2L^2\gamma^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E}\left\|\u_{t-1} \right\|^2 + \frac{360\omega^2\alpha^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{360\omega^2\alpha^2(\sigma^2 + \zeta^2)T}{(1-15\omega^2)(1-12\omega^2)}\\
% &+ \frac{1200\omega^2\alpha^2 + 480\omega^2L^2\gamma^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2
% \end{align*}
% If we can guarantee that $(1200\omega^2\alpha^2 + 480\omega^2L^2\gamma^2)\leq  \frac{(1-15\omega^2)(1-12\omega^2)}{2}$,
% then we have
% \begin{align*}
% &\sum_{t=0}^{T-1}\mathbb{E}\|\odelta_t\|^2\\
% \leq & \frac{480\omega^2L^2\gamma^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E}\left\|\u_{t-1} \right\|^2 + \frac{720\omega^2\alpha^2}{(1-15\omega^2)(1-12\omega^2)}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{720\omega^2\alpha^2(\sigma^2 + \zeta^2)T}{(1-15\omega^2)(1-12\omega^2)}.
% \end{align*}
% \end{proof}




\section{Proof of Theorem~\ref{theo:general_nonconvex}}
\begin{proof}
In the view of $\{\hat{\x}_t\}$, we have
\begin{align*}
&\mathbb{E} f(\hat{\x}_{t+1}) - \mathbb{E} f(\hat{\x}_t)\\
\leq & \mathbb{E} \langle \nabla f(\hat{\x}_t), \hat{\x}_{t+1} - \hat{\x}_t \rangle + \frac{L}{2}\mathbb{E}\|\hat{\x}_{t+1} - \hat{\x}_t\|^2\\
= & -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t), \u_t \rangle + \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2\\
= & -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t), \hat{\u}_{t} + (\u_t - \hat{\u}_{t}) \rangle + \frac{L\gamma^2}{2}\mathbb{E}\|\hat{\u}_{t} + (\u_t - \hat{\u}_{t})\|^2\\
\leq & -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t), \hat{\u}_{t}\rangle -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t), \u_t - \hat{\u}_{t} \rangle + L\gamma^2\mathbb{E}\|\hat{\u}_{t}\|^2 + L\gamma^2\mathbb{E}\|\u_t - \hat{\u}_{t}\|^2\\
\leq & -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t), \hat{\u}_{t}\rangle +\frac{\gamma}{4}\mathbb{E} \| \nabla f(\hat{\x}_t)\|^2 + \gamma\E\| \u_t - \hat{\u}_{t} \|^2 + L\gamma^2\mathbb{E}\|\hat{\u}_{t}\|^2 + L\gamma^2\mathbb{E}\|\u_t - \hat{\u}_{t}\|^2\\
\leq & -\frac{\gamma}{2}\left(\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2 + \E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2\right) +\frac{\gamma}{4}\mathbb{E} \| \nabla f(\hat{\x}_t)\|^2\\
&+ \gamma\| \u_t - \hat{\u}_{t} \|^2 + L\gamma^2\mathbb{E}\|\hat{\u}_{t}\|^2 + L\gamma^2\mathbb{E}\|\u_t - \hat{\u}_{t}\|^2\\
\leq & -\frac{\gamma}{8}\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2 - \frac{\gamma}{2}\left((1-2L\gamma)\E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2 + \frac{\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2}{4}\right) + (1 + L\gamma)\gamma\E\| \u_t - \hat{\u}_{t} \|^2.
\end{align*}
Summing up the inequality above from $t=0$ to $t=T$, with rearrangement we get
\begin{align*}
&\frac{1}{T}\sum_{t=0}^T\E\|\nabla f(\hat{\x}_t)\|^2\\
\leq & \frac{8(f(\hat{\x}_0) - f(\hat{\x}_{T+1}))}{\gamma T} - \frac{4}{T}\sum_{t=0}^T\left((1-2L\gamma)\E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2+ \frac{\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2}{4}\right)\\
&+ \frac{8+ 8L\gamma}{T}\sum_{t=0}^T\E\| \u_t - \hat{\u}_{t} \|^2\\
\leq & \frac{8(f(\x_0) - f^*)}{\gamma T} - \frac{4}{T}\sum_{t=0}^T\left((1-2L\gamma)\E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2+ \frac{\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2}{4}\right)\\
&+ \frac{8 + 8L\gamma}{T}\sum_{t=0}^T\E\| \u_t - \hat{\u}_{t} \|^2.\numberthis\label{proof:theo_y_t:eq1}
\end{align*}
In order to upper bound $\E\| \u_t - \hat{\u}_{t} \|^2$, we have
\begin{align*}
&\E\| \u_t - \hat{\u}_{t} \|^2\\
=& \E\| (1-\alpha)(\u_{t-1} - \hat{\u}_{t-1}) + \alpha(\A(\x_t;\xi_t) - \A(\hat{\x}_t;\xi_t))  \|^2\\
\leq & \left( 1 + \alpha\right)\E\| (1-\alpha)(\u_{t-1} - \hat{\u}_{t-1})\|^2 +  \left(1+ \frac{1}{\alpha} \right)\E\|\alpha(\A(\x_t;\xi_t) - \A(\hat{\x}_t;\xi_t))  \|^2\\
= & \left( 1 - \alpha^2\right)(1-\alpha)\E\| \u_{t-1} - \hat{\u}_{t-1}\|^2 +  \left(\alpha^2+\alpha \right)\E\|\A(\x_t;\xi_t) - \A(\hat{\x}_t;\xi_t)  \|^2\\
\leq & \left( 1 - \alpha\right)\E\| \u_{t-1} - \hat{\u}_{t-1}\|^2 +  2\alpha\E\|\A(\x_t;\xi_t) - \A(\hat{\x}_t;\xi_t)  \|^2\\
= & (1-\alpha)^t\E\| \u_{0} - \u_{0}(\y)\|^2 + 2\alpha\sum_{s=0}^t(1-\alpha)^{t-s}\E\|\A(\x_s;\xi_s) - \A(\hat{\x}_s;\xi_s)  \|^2\\
= &  2\alpha\sum_{s=0}^t(1-\alpha)^{t-s}\E\|\A(\x_s;\xi_s) - \A(\hat{\x}_s;\xi_s)  \|^2\quad\text{($\u_{0} - \u_{0}(\y) = \bm{0}$)}\\
\leq & 2\alpha L^2_{\A}\sum_{s=0}^t(1-\alpha)^{t-s}\E\|\x_s - \hat{\x}_s \|^2.
\end{align*}
Therefore we have
\begin{align*}
\sum_{t=0}^T \E\| \u_t - \hat{\u}_{t} \|^2\leq & 2\alpha L^2_{\A}\sum_{t=0}^T\sum_{s=0}^t(1-\alpha)^{t-s}\E\|\x_s - \hat{\x}_s \|^2\\
= & 2\alpha L^2_{\A}\sum_{s=0}^T\sum_{t=s}^T(1-\alpha)^{t-s}\E\|\x_s - \hat{\x}_s \|^2\\
\leq & 2 L^2_{\A}\sum_{t=0}^T\E\|\x_t - \hat{\x}_t \|^2.\numberthis\label{proof:theo_y_t:eq2}
\end{align*}
Combining \eqref{proof:theo_y_t:eq1} and \eqref{proof:theo_y_t:eq2} together we get
\begin{align*}
&\frac{1}{T}\sum_{t=0}^T\E\|\nabla f(\hat{\x}_t)\|^2\\
\leq & \frac{8(f(\x_0) - f^*)}{\gamma T} - \frac{4}{T}\sum_{t=0}^T\left((1-2L\gamma)\E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2+ \frac{\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2}{4}\right)\\
&+ \frac{16(1 + L\gamma) L^2_{\A}}{T}\sum_{t=0}^T\E\|\x_t - \hat{\x}_t \|^2.
\end{align*}
Hence $\|\nabla f(\x_t)\|^2$ can be upper bounded by using 
\begin{align*}
&\frac{1}{T}\sum_{t=0}^T\E\|\nabla f(\x_t)\|^2\\
\leq & \frac{1}{T}\sum_{t=0}^T\E\|\nabla f(\hat{\x}_t) + (\nabla f(\x_t) - \nabla f(\hat{\x}_t))\|^2\\
\leq & \frac{2}{T}\sum_{t=0}^T\E\|\nabla f(\hat{\x}_t)\|^2 + \frac{2}{T}\sum_{t=0}^T\E\|\nabla f(\x_t) - \nabla f(\hat{\x}_t)\|^2\\
\leq & \frac{2}{T}\sum_{t=0}^T\E\|\nabla f(\hat{\x}_t)\|^2 + \frac{2L^2}{T}\sum_{t=0}^T\E\|\x_t - \hat{\x}_t\|^2\\
\leq & \frac{16(f(\x_0) - f^*)}{\gamma T} - \frac{8}{T}\sum_{t=0}^T\left((1-2L\gamma)\E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2+ \frac{\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2}{4}\right)\\
&+ \frac{ 32(1 + L\gamma) L^2_{\A} + 2L^2}{T}\sum_{t=0}^T\E\| \u_t - \hat{\u}_{t} \|^2.
\end{align*}
If $L\gamma \leq 1$, then we have
\begin{align*}
&\frac{1}{T}\sum_{t=0}^T\E\|\nabla f(\x_t)\|^2\\
\leq & \frac{16(f(\x_0) - f^*)}{\gamma T} - \frac{8}{T}\sum_{t=0}^T\left((1-2L\gamma)\E\|\hat{\u}_{t}\|^2 - \E\|\nabla f(\hat{\x}_t) - \hat{\u}_{t}\|^2 +\frac{\mathbb{E} \|\nabla f(\hat{\x}_t)\|^2}{4}\right)\\ 
 &+ \frac{64 L^2_{\A} + 2L^2}{T}\sum_{t=0}^T\E\|\x_t - \hat{\x}_t \|^2,
\end{align*}
which completes the proof.
\end{proof}


\section{Proof to Theorem~\ref{theo:general_strongly}}

\begin{lemma}\label{strongly:seq_lemma}
For any sequence that satisfies
\begin{align*}
a_{t+1} \leq& (1-\beta\gamma_t)a_t - \gamma_t s_t + \gamma_t^2 c_t;\\
0< & \gamma_t\leq  \gamma_{\max},
\end{align*}
where $\gamma_{\max}$ is a constant. Setting $\gamma_t=\frac{2}{\beta(\kappa + t)}$ where $\kappa = \frac{2}{\gamma_{\max}\beta}$, then we have
\begin{align*}
\sum_{t=1}^T(\kappa+t)s_t + \frac{\beta(\kappa + T)^2a_{T+1}}{2}\leq   \frac{\beta\kappa^2a_{1}}{2} +  \frac{2}{\beta}\sum_{t=1}^Tc_t.
\end{align*}
\end{lemma}

\begin{proof}
Defining $w_t = (\kappa + t)$, we have
\begin{align*}
\frac{w_ta_{t+1}}{\gamma_t} \leq \frac{(1-\beta\gamma_t)w_ta_t}{\gamma_t} - w_ts_t + w_t\gamma_t c_t;\\
\frac{(\kappa +t)^2\beta a_{t+1}}{2} \leq \frac{(1-\beta\gamma_t)w_ta_t}{\gamma_t} - w_ts_t +  w_t\gamma_t c_t.
\end{align*}
Notice that
\begin{align*}
\frac{(1-\beta\gamma_t)w_t}{\gamma_t} =& \frac{(1-\beta\gamma_t)\beta(\kappa + t)^2}{2}\\
= & \left(1-\frac{2}{\kappa + t} \right)\frac{\beta(\kappa + t)^2}{2}\\
= & \frac{\beta(\kappa + t)(\kappa +t -2)}{2}\\
\leq & \frac{\beta(\kappa +t -1)^2}{2},
\end{align*}
which leads to
\begin{align*}
\frac{(\kappa +t)^2\beta a_{t+1}}{2} \leq& \frac{\beta(\kappa +t -1)^2}{2}a_t - w_ts_t +  w_t\gamma_t c_t;\\
w_ts_t\leq & \frac{\beta}{2}\left((\kappa +t -1)^2a_{t} - (\kappa + t)^2a_{t+1}  \right) + \frac{2c_t}{\beta}.
\end{align*}
Summing up the inequality above from $t=1$ to $t=T$ we get
\begin{align*}
&\sum_{t=1}^Tw_ts_t\leq  -\frac{\beta(\kappa + T)^2a_{T+1}}{2} +\frac{\beta\kappa^2a_{1}}{2} +  \frac{2}{\beta}\sum_{t=1}^Tc_t;\\
&\sum_{t=1}^Tw_ts_t + \frac{\beta(\kappa + T)^2a_{T+1}}{2}\leq   \frac{\beta\kappa^2a_{1}}{2} +  \frac{2}{\beta}\sum_{t=1}^Tc_t.
\end{align*}
\end{proof}



\begin{lemma}\label{strongly:seq_lemma_2}
For any sequence that satisfies
\begin{align*}
a_{t+1} \leq& (1-\alpha_t)a_t + b_t,
\end{align*}
For any positive sequence $\gamma_t$, if $\alpha_t \geq 1- \frac{\gamma_{t-1}}{\gamma_t}$, then we have
\begin{align*}
\sum_{t=1}^Tw_ts_t + \frac{\beta(\kappa + T)^2a_{T+1}}{2}\leq   \frac{\beta\kappa^2a_{1}}{2} +  \frac{2}{\beta}\sum_{t=1}^Tc_t.
\end{align*}
\end{lemma}

\begin{proof}
Since
\begin{align*}
\frac{a_{t+1}}{\gamma_{t+1}}\leq &\frac{a_t}{\gamma_t} + \frac{b_t}{\gamma_{t+1}} + \frac{a_t}{\gamma_t}\left(\frac{(1-\alpha_t)\gamma_t}{\gamma_{t-1}} - 1  \right)\\
\leq & \frac{a_t}{\gamma_t} + \frac{b_t}{\gamma_{t+1}}.
\end{align*}
Summing up the inequality above from $t=1$ to $t=T$ we get
\begin{align*}
\frac{a_{T+1}}{\gamma_{T+1}} \leq \frac{a_1}{\gamma_1} \sum_{t=1}^T\frac{b_t}{\gamma_{t+1}},
\end{align*}
which completes the proof
\end{proof}




Now we are ready to present the proof of Theorem XXX.
\begin{proof}
For $\{\hat{\x}_t\}$, we have
\begin{align*}
&\E\|\hx_{t+1} - \x^*\|^2\\
= & \E\|\hx_t - \x^*\|^2 + 2\E\langle \hx_t - \x^*, \hx_{t+1} - \hx_{t}\rangle + \E\|\hx_{t+1} - \hx_{t}\|^2\\
= & \E\|\hx_t - \x^*\|^2 - 2\gamma_t\E\langle \hx_t - \x^*, \u_t\rangle + \gamma_t^2\E\|\u_t\|^2\\
= & \E\|\hx_t - \x^*\|^2 - 2\gamma_t\E\langle \hx_t - \x^*, \nabla f(\hx_t)\rangle + 2\gamma_t\E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \gamma_t^2\E\|\u_t\|^2\\
\leq & \E\|\hx_t - \x^*\|^2 - 2\gamma_t\left( \frac{\mu}{2}\E\|\hx_t - \x^*\|^2 + \E f(\hx_t) - f^* \right) + 2\gamma_t\E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \gamma_t^2\E\|\u_t\|^2\\
= & \left(1-{\mu\gamma_t}  \right)\E\|\hx_t - \x^*\|^2 - 2\gamma_t\left(  \E f(\hx_t) - f^* \right) +2\gamma_t\E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \gamma_t^2\E\|\u_t\|^2\\
\leq & \left(1-{\mu\gamma_t}  \right)\E\|\hx_t - \x^*\|^2 - 2\gamma_t\left(  \E f(\hx_t) - f^* \right) +2\gamma_t\E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle\\
&+ 2\gamma_t^2\E\|\nabla f(\hx_t) -\u_t\|^2 + 2\gamma_t^2 \E\|\nabla f(\hx_t)\|^2.\numberthis\label{strongly:general_eq1}
\end{align*}
Notice that we have
\begin{align*}
f(\x) - f^*\geq & f(\x) - f\left(\x - \frac{1}{L}\nabla f(\x)\right)\\
\geq & f(\x) - \left(f(\x) - \frac{1}{L}\|\nabla f(\x)\|^2 + \frac{L}{2L^2}\|\nabla f(\x)\|^2\right)\\
= & \frac{1}{2L}\|\nabla f(\x)\|^2.
\end{align*}
Therefore \eqref{strongly:general_eq1} becomes
\begin{align*}
&\E\|\hx_{t+1} - \x^*\|^2\\
\leq &\left(1-{\mu\gamma_t}  \right)\E\|\hx_t - \x^*\|^2 - \frac{2\gamma_t(1-\gamma_t L)}{L}\E\|\nabla f(\hx_t)\|^2  +2\gamma_t\E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle\\
&+ 2\gamma_t^2\E\|\nabla f(\hx_t) -\u_t\|^2.\numberthis\label{proof:strongly_induction_xt}
\end{align*}
Next we need to give an upper bound for $\E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle$, we first expand it as
\begin{align*}
&\E\langle \hx_{t+1} - \x^*, \nabla f(\hx_{t+1}) - \u_{t+1}\rangle\\
= & \E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \E\langle \hx_{t+1} - \hx_t, \nabla f(\hx_{t}) - \u_{t}\rangle\\
&+ \E\langle \hx_{t} - \x^*, \nabla f(\hx_{t+1}) - \u_{t+1}- \nabla f(\hx_t) + \u_t\rangle + \E\langle \hx_{t+1} - \hx_t, \nabla f(\hx_{t+1}) - \u_{t+1}- \nabla f(\hx_t) + \u_t\rangle\\
= &  \E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle - \gamma_t\E\langle \u_t, \nabla f(\hx_{t}) - \u_{t}\rangle\\
&+ \E\langle \hx_{t} - \x^*, \nabla f(\hx_{t+1}) - \u_{t+1}- \nabla f(\hx_t) + \u_t\rangle - \gamma_t\E\langle \u_t, \nabla f(\hx_{t+1}) - \u_{t+1}- \nabla f(\hx_t) + \u_t\rangle.\numberthis\label{proof:strongly_induction_dot_eq1}
\end{align*}
For $\nabla f(\hx_{t+1}) - \u_{t+1}- \nabla f(\hx_t) + \u_t$, we have
\begin{align*}
&\nabla f(\hx_{t+1}) - \u_{t+1}- \nabla f(\hx_t) + \u_t\\
=& \nabla f(\hx_{t+1}) - (1-\alpha_{t+1})\u_{t} - \alpha_{t+1}\b_{t+1}- \nabla f(\hx_t) + \u_t\\
= & -\alpha_{t+1}(\nabla f(\hx_t) - \u_t) + \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t}).\numberthis\label{proof:strongly_induction_dot_eq2}
\end{align*}
Combing \eqref{proof:strongly_induction_dot_eq1} and \eqref{proof:strongly_induction_dot_eq2} we get
\begin{align*}
&\E\langle \hx_{t+1} - \x^*, \nabla f(\hx_{t+1}) - \u_{t+1}\rangle\\
= & (1-\alpha_{t+1}) \E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \E\langle \hx_{t} - \x^*, \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
& - \gamma_t\E\langle \u_t, \nabla f(\hx_{t}) - \u_{t}\rangle - \gamma_t\E\langle \u_t, \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
= & (1-\alpha_{t+1}) \E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \E\langle \hx_{t} - \x^*, \nabla f(\hx_{t+1}) - \alpha_{t+1}\E_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
& - \gamma_t\E\langle \u_t, \nabla f(\hx_{t}) - \u_{t}\rangle - \gamma_t\E\langle \u_t, \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
\leq & (1-\alpha_{t+1}) \E\langle \hx_t - \x^*, \nabla f(\hx_t) - \u_t\rangle + \E\langle \hx_{t} - \x^*, \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
& - \gamma_t\E\langle \u_t, \nabla f(\hx_{t}) - \u_{t}\rangle - \gamma_t\E\langle \u_t, \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
\leq & (1-\alpha_{t+1}) \E\| \hx_t - \x^*, \nabla f(\hx_t) - \u_t\|^2 + \frac{\mu\alpha_{t+1}}{32}\E\| \hx_{t} - \x^*\|^2\\
&+ \frac{16}{\mu\alpha_{t+1}}\E\| \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\|^2\\
& - \gamma_t\E\langle \u_t, \nabla f(\hx_{t}) - \u_{t}\rangle - \gamma_t\E\langle \u_t, \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\rangle\\
\leq & (1-\alpha_{t+1}) \E\| \hx_t - \x^*, \nabla f(\hx_t) - \u_t\|^2 + \frac{\mu\alpha_{t+1}}{32}\E\| \hx_{t} - \x^*\|^2\\
&+ \frac{16}{\mu\alpha_{t+1}}\E\| \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\|^2\\
& + \frac{\gamma_t\E\| \u_t\|^2}{2} + \frac{\gamma_t\E\|\nabla f(\hx_{t}) - \u_{t}\|^2}{2} +  \frac{\gamma_t\E\| \u_t\|^2}{2} + \frac{\gamma_t\E\|\nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\|^2}{2}\\
\leq & (1-\alpha_{t+1}) \E\| \hx_t - \x^*, \nabla f(\hx_t) - \u_t\|^2 + \frac{\mu\alpha_{t+1}}{32}\E\| \hx_{t} - \x^*\|^2+ 3\gamma_t\E\|\nabla f(\hx_{t}) - \u_{t}\|^2 +  2\gamma_t\E\| \nabla f(\hx_t)\|^2\\
&+ \left(\frac{16}{\mu\alpha_{t+1}} + \frac{\gamma_t}{2}\right)\E\| \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t})\|^2.\numberthis\label{proof:strongly_induction_dot}
\end{align*}
Combining \eqref{proof:strongly_induction_dot} and \eqref{proof:strongly_induction_xt} together, and defining 
\begin{align*}
Y_t :=&\left(\begin{array}{l}
    \E\|\hx_{t+1} - \x^*\|^2 \\
     \E\langle \hx_{t+1} - \x^*,\nabla f(\hx_{t+1}) - \u_{t+1}\rangle
\end{array}   \right),\\
\Lambda_t :=&\left(\begin{array}{cc}
   1-\mu\gamma_t  & 2\gamma_t \\
   \frac{\mu\alpha_{t+1}}{32}  & 1-\alpha_{t+1}
\end{array}\right),\\
\bm{r_t}:= & \nabla f(\hx_{t+1}) - \alpha_{t+1}\b_{t+1} - (1-\alpha_{t+1})f(\hx_{t}),\\
Z_t :=& \left(\begin{array}{l}
 - \frac{2\gamma_t(1-\gamma_t L)}{L}\E\|\nabla f(\hx_t)\|^2 + 2\gamma_t^2\E\|\nabla f(\hx_t) -\u_t\|^2      \\
      3\gamma_t\E\|\nabla f(\hx_{t}) - \u_{t}\|^2 +  2\gamma_t\E\| \nabla f(\hx_t)\|^2+ \left(\frac{16}{\mu\alpha_{t+1}} + \frac{\gamma_t}{2}\right)\E\|\bm{r}_t \|^2
\end{array}
\right)
\end{align*}
we have
\begin{align*}
Y_{t+1}\leq \Lambda_t Y_t + Z_t.\numberthis\label{proof:strongly_induction_matrix}
\end{align*}
It can be easily verified that the eigenvalue of $Z_t$ are
\begin{align*}
\lambda_{1,t} = 1- \frac{\mu\gamma_t + \alpha_{t+1}}{2} + \frac{\|\mu\gamma_t - \alpha_{t+1}\|\sqrt{1+ \frac{\mu\gamma_t\alpha_{t+1}}{4(\mu\gamma_t - \alpha_{t+1})^2}}}{2},\\
\lambda_{2,t} = 1- \frac{\mu\gamma_t + \alpha_{t+1}}{2} - \frac{\|\mu\gamma_t - \alpha_{t+1}\|\sqrt{1+ \frac{\mu\gamma_t\alpha_{t+1}}{4(\mu\gamma_t - \alpha_{t+1})^2}}}{2}.
\end{align*}
Therefore if $\alpha_{t+1}\geq 2\mu\gamma_t$, then we can ensure that
\begin{align*}
\lambda_{1,t} \leq & 1- \mu\gamma_t + \frac{(\alpha_{t+1} - \mu\gamma_t)\left(\sqrt{1+ \frac{\mu\gamma_t\alpha_{t+1}}{4(\mu\gamma_t - \alpha_{t+1})^2}} - 1\right)}{2}\\
\leq & 1- \mu\gamma_t + \frac{\frac{\alpha_{t+1}}{2}\left(\sqrt{1+\frac{\mu\gamma_t}{\alpha_{t+1}} } - 1\right)}{2}\\
\leq & 1- \mu\gamma_t + \frac{\mu\gamma_t}{8}\\
\leq & 1-\frac{\mu\gamma_t}{2}.
\end{align*}



\newpage
If $\gamma_t \leq \frac{1}{4L}$, then we have
\begin{align*}
\E\|\hx_{t+1} - \x^*\|^2\leq & \left(1-\frac{\mu\gamma_t}{2}  \right)\E\|\hx_t - \x^*\|^2 - \gamma_t\left(  \E f(\hx_t) - f^* \right)  +\left(\frac{2\gamma_t}{\mu} + 2\gamma_t^2 \right)\E \|\nabla f(\hx_t) - \u_t\|^2\\
\leq &\left(1-\frac{\mu\gamma_t}{2}  \right)\E\|\hx_t - \x^*\|^2 - \gamma_t\left(  \E f(\hx_t) - f^* \right)  +2\left(\frac{2\gamma_t}{\mu} + 2\gamma_t^2 \right)\E \|\nabla f(\hx_t) - \hu_t\|^2\\ 
&+ 2\left(\frac{2\gamma_t}{\mu} + 2\gamma_t^2 \right)\E \|\u_t - \hu_t\|^2\\
\leq &\left(1-\frac{\mu\gamma_t}{2}  \right)\E\|\hx_t - \x^*\|^2 - \gamma_t\left(  \E f(\hx_t) - f^* \right)  +2\left(\frac{2\gamma_t}{\mu} + 2\gamma_t^2 \right)\E \|\nabla f(\hx_t) - \hu_t\|^2\\ 
&+ 4L_{\A}\left(\frac{2\gamma_t}{\mu} + 2\gamma_t^2 \right)\E \|\x_t - \hx_t\|^2. \text{\yl refer to (14), this holds in sum}
\numberthis\label{strongly:general_eq2}
\end{align*}
If $\gamma_t\leq \frac{1}{\mu}$, then \eqref{strongly:general_eq2} becomes
\begin{align*}
\E\|\hx_{t+1} - \x^*\|^2\leq & \left(1-\frac{\mu\gamma_t}{2}  \right)\E\|\hx_t - \x^*\|^2 - \gamma_t\left(  \E f(\hx_t) - f^* \right)  +\frac{8\gamma_t^2}{\mu}\frac{\E \|\nabla f(\hx_t) - \hu_t\|^2}{\gamma_t}+ \frac{16\gamma_t^2L_{\A}}{\mu} \frac{\E \|\x_t - \hx_t\|^2}{\gamma_t}
\end{align*}
By using Lemma~\ref{strongly:seq_lemma}, setting $\gamma_t = \frac{4}{\mu\left(\frac{4L}{\mu} + t \right)}$ the inequality above leads to
\begin{align*}
\left(\frac{4L}{\mu} + T \right)^2\E\|\hx_{T+1} - \x^*\|^2\leq & \frac{4L^2}{\mu}\E\|\hx_{1} - \x^*\|^2 + \frac{96\left(\frac{4L}{\mu} + T \right)}{\mu^2}\sum_{t=1}^T\left(\E \|\nabla f(\hx_t) - \hu_t\|^2 + 2L_\A\E \|\x_t - \hx_t\|^2  \right);\\
\E\|\hx_{T+1} - \x^*\|^2\leq & \frac{4L^2}{\mu T^2}\E\|\hx_{1} - \x^*\|^2 + \frac{96}{\mu^2\left(\frac{4L}{\mu} + T \right)}\sum_{t=1}^T\left(\E \|\nabla f(\hx_t) - \hu_t\|^2 + 2L_\A\E \|\x_t - \hx_t\|^2  \right).\numberthis\label{strongly:general_eq3}
\end{align*}
The upper bound for $\E\|\x_T - \x^*\|^2$ can be estimated using
\begin{align*}
\E\|\x_T - \x^*\|^2\leq & 2\E\|\hx_T - \x^*\|^2 + 2\E\|\hx_T - \x_T\|^2,
\end{align*}
which, by using \eqref{strongly:general_eq3}, we have
\begin{align*}
\E\|\x_T - \x^*\|^2\leq & \frac{8L^2}{\mu T^2}\E\|\hx_{1} - \x^*\|^2 + \frac{192}{\mu^2\left(\frac{4L}{\mu} + T \right)}\sum_{t=1}^T\left(\E \|\nabla f(\hx_t) - \hu_t\|^2 + 2L_A\E \|\x_t - \hx_t\|^2  \right) + 2\E\|\hx_T - \x_T\|^2.
\end{align*}
\end{proof}

\newpage
% \begin{lemma}\label{lemma:general_step1}
% For any algorithm that follows the updating rule of \eqref{update:general_compress}, we have the following convergence rate
% \begin{align*}
% &\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2 + \frac{1 }{2 T}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbb E_t\u_t\|^2 \\
% \leq & \frac{2(f(\x_{0}) - f^*)}{\gamma T}  + \frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2 + \frac{8L^2}{T}\sum_{t=0}^{T-1}\mathbb E\|\hat{\x}_t - \x_t\|^2 + \frac{1}{T}\sum_{t=1}^{T-1}\mathbb E\|\u_t\|^2.
% \end{align*}
% \end{lemma}
% Instead of investigating $\{\x_t\}$ directly, here we  $\{\hat{\x}_t\}$ that follows the updating rule of
% \begin{align*}
% \hat{\x}_{t+1} = \hat{\x}_t - \gamma \u_t.
% \end{align*}
% Then we have
% \begin{align*}
% &\mathbb{E} f(\hat{\x}_{t+1}) - \mathbb{E} f(\hat{\x}_t)\\
% \leq & \mathbb{E} \langle \nabla f(\hat{\x}_t), \hat{\x}_{t+1} - \hat{\x}_t \rangle + \frac{L}{2}\mathbb{E}\|\hat{\x}_{t+1} - \hat{\x}_t\|^2\\
% = & -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t), \u_t \rangle + \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2\\
% = & -\gamma\mathbb{E} \langle \nabla f(\hat{\x}_t) -\nabla f(\x_t) + \nabla f(\x_t),  \u_t  \rangle + \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2\\
% \leq & \gamma\left( 4\mathbb{E}\left\| \nabla f(\hat{\x}_t) -\nabla f(\x_t)\right\|^2  + \frac{1}{4}\mathbb{E}\|\u_t\|^2 - \mathbb{E} \langle  \nabla f(\x_t),  \mathbb E_t\u_t  \rangle      \right)+ \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2\\
% \leq & \gamma\left( 4\mathbb{E}\left\| \nabla f(\hat{\x}_t) -\nabla f(\x_t)\right\|^2  + \frac{1}{4}\mathbb{E}\|\mathbb E_t\u_t\|^2 - \frac{\mathbb{E}\|\nabla f(\x_t)\|^2 + \mathbb{E}\|\mathbb E_t\u_t\|^2 - \mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2  }{2}\right)+ \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2\\
% \leq & -\frac{\gamma}{2}\mathbb{E}\|\nabla f(\x_t)\|^2 - \frac{\gamma }{4}\mathbb{E}\|\mathbb E_t\u_t\|^2 + 4\gamma\mathbb{E}\left\| \nabla f(\hat{\x}_t) -\nabla f(\x_t)\right\|^2 + \frac{\gamma}{2}\mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2 + \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2\\
% \leq & -\frac{\gamma}{2}\mathbb{E}\|\nabla f(\x_t)\|^2 - \frac{\gamma}{4}\mathbb{E}\|\mathbb E_t\u_t\|^2 + 4\gamma L^2\mathbb{E}\left\| \hat{\x}_t - \x_t\right\|^2 + \frac{\gamma}{2}\mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2 + \frac{L\gamma^2}{2}\mathbb{E}\|\u_t\|^2.
% \end{align*}
% Summing up the inequality above from $t=0$ to $t=T-1$, with rearrangement we get
% \begin{align*}
% &\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2 + \frac{1 }{2 T}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbb E_t\u_t\|^2 \\
% \leq&  \frac{2(f(\hat{\x}_{0}) - \mathbb{E} f(\hat{\x}_T))}{\gamma T}  + \frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2 + \frac{8L^2}{T}\sum_{t=0}^{T-1}\mathbb E\|\hat{\x}_t - \x_t\|^2 + \frac{\gamma}{T}\sum_{t=1}^{T-1}\mathbb E\|\u_t\|^2\\
% \leq & \frac{2(f(\x_{0}) - f^*)}{\gamma T}  + \frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2 + \frac{8L^2}{T}\sum_{t=0}^{T-1}\mathbb E\|\hat{\x}_t - \x_t\|^2 + \frac{\gamma}{T}\sum_{t=1}^{T-1}\mathbb E\|\u_t\|^2.
% \end{align*}

\subsection{Proof to Theorem~\ref{theo:main}}
In this section, we are going to present the proof to STORM-\CR start with some key lemmas.
\begin{lemma}\label{lemma:contraction}
For any sequence $\{a_t\}$ and $\{b_t\}$ that satisfies
\begin{align*}
a_t\leq \rho a_{t-1} + b_t,
\end{align*}
where $\rho$ is a constant satisfies $0<\rho<1$, we have
\begin{align*}
\sum_{t=0}^{T}a_t\leq \frac{\sum_{t=1}^{T}b_t + a_0}{1-\rho}.
\end{align*}
\end{lemma}
\begin{proof}
Since 
\begin{align*}
a_t\leq \rho a_{t-1} + b_t,
\end{align*}
adding the inequality above from $t=1$ to $t=T$ we get
\begin{align*}
\sum_{t=1}^{T}a_t \leq& \rho\sum_{t=0}^{T-1}a_t + \sum_{t=1}^{T}b_t\\
\leq & \rho\sum_{t=0}^{T}a_t + \sum_{t=1}^{T}b_t.
\end{align*}
Adding $a_0$ to both side we get
\begin{align*}
\sum_{t=0}^{T}a_t\leq & \rho\sum_{t=0}^{T}a_t + \sum_{t=1}^{T}b_t + a_0.
\end{align*}
\end{proof}

\begin{lemma}
For Momentum SGD (without compression), if $\gamma\leq \frac{\alpha}{8L}$, then we have
\begin{align*}
\sum_{t=0}^TA_t \leq 6\gamma L\sigma^2T.
\end{align*}
\end{lemma}
\begin{proof}
For \textbf{Momentum SGD}, denote $\m_t = \alpha\sum_{t=0}^t(1-\alpha) \nabla f(\x_s)$, then we have
\begin{align*}
&\E\|\nabla f(\x_t) - \u_{t}\|^2 - \E\|\u_{t}\|^2\\
=& \E\|\nabla f(\x_t)\|^2 - 2\E\langle \nabla f(\x_t),\u_t\rangle\\
= &\E\|\nabla f(\x_t)\|^2 - 2\E\langle \nabla f(\x_t),\m_t\rangle - 2\E\langle \nabla f(\x_t),\u_t - \m_t\rangle\\
= &\E\|\nabla f(\x_t)\|^2 - 2\E\langle \nabla f(\x_t),\m_t\rangle - 2\E\langle \nabla f(\x_t),\u_t - \m_t\rangle\\
= & -\E\|\m_t\|^2 + \E\|\nabla f(\x_t) - \m_t\|^2- 2\E\langle \nabla f(\x_t),\u_t - \m_t\rangle.\numberthis\label{lemma:momentum_eq0}
\end{align*}
For $\E\|\nabla f(\x_t) - \m_t\|^2$ we have
\begin{align*}
&\E\|\nabla f(\x_t) - \m_t\|^2\\
\leq & \E\|(1-\alpha)(\nabla f(\x_{t-1}) - \m_{t-1} + \nabla f(\x_t) - \nabla f(\x_{t-1}))\|^2\\
\leq & \left((1-\alpha)^2 + \alpha\right)\E\|\nabla f(\x_{t-1}) - \m_{t-1}\|^2 + \frac{1}{\alpha}\E\|\nabla f(\x_t) - \nabla f(\x_{t-1}))\|^2\\
\leq & (1-\alpha)\E\|\nabla f(\x_{t-1}) - \m_{t-1}\|^2 + \frac{L^2\gamma^2}{\alpha}\E\|\m_t\|^2.
\end{align*}
Therefore we have
\begin{align*}
\sum_{t=0}^T\E\|\nabla f(\x_t) - \m_t\|^2 \leq & \frac{L^2\gamma^2}{\alpha^2}\sum_{t=0}^T\E\|\m_t\|^2.\numberthis\label{lemma:momentum_eq1}
\end{align*}
For $\E\langle \nabla f(\x_t),\u_t - \m_t\rangle$, we have
\begin{align*}
&\E\left\langle \nabla f(\x_t), \u_t - \m_t\right\rangle\\
=& \E\left\langle \nabla f(\x_{t}), (1-\alpha)(\u_{t-1} - \m_{t-1})+ \alpha(\g_t - \nabla f(\x_t)  )  \right\rangle\\
=& \E\left\langle \nabla f(\x_{t}), (1-\alpha)(\u_{t-1} - \m_{t-1}) \right\rangle\\
= & (1-\alpha)\E\left\langle \nabla f(\x_{t-1}), \u_{t-1} - \m_{t-1}  \right\rangle + (1-\alpha)\E\left\langle \nabla f(\x_{t}) - \nabla f(\x_{t-1}), \u_{t-1} - \m_{t-1}  \right\rangle.\numberthis\label{lemma:momentum_eq2}
\end{align*}

Notice that for $\nabla f(\x_{t}) - \nabla f(\x_{t-1}) $, we have
\begin{align*}
&\E\left\|\nabla f(\x_{t}) - \nabla f(\x_{t-1}) \right\|^2\\
\leq & L^2\gamma^2\E\|\u_{t-1} - \m_{t-1} + \m_{t-1}\|^2\\
\leq & 2L^2\gamma^2\E\| \m_{t-1}\|^2+2L^2\gamma^2\E\|\u_{t-1} - \m_{t-1}\|^2 .\numberthis\label{lemma:momentum_eq3}
\end{align*}
Combining \eqref{lemma:momentum_eq2} and \eqref{lemma:momentum_eq3} together we get
\begin{align*}
&\E\left\langle \nabla f(\x_t), \u_t - \m_t\right\rangle\\
\leq & (1-\alpha)\E\left\langle \nabla f(\x_{t-1}), \u_{t-1} - \m_{t-1}  \right\rangle + (1-\alpha)\E\left( \frac{1}{\gamma L}\left\|\nabla f(\x_{t}) - \nabla f(\x_{t-1}) \right\|^2 + \gamma L\E\left\| \u_{t-1} - \m_{t-1}  \right\|^2\right)\\
\leq & (1-\alpha)\E\left\langle \nabla f(\x_{t-1}), \u_{t-1} - \m_{t-1}  \right\rangle + (1-\alpha)\E\left( \gamma L\E\| \m_{t-1}\|^2 +3\gamma\E\left\| \u_{t-1} - \m_{t-1}  \right\|^2\right),
\end{align*}


Denote $c_t:=2\gamma L\E\| \m_{t-1}\|^2 +3\gamma\E\left\| \u_{t-1} - \m_{t-1}  \right\|^2$, from the equation above we get
\begin{align*}
\E\left\langle \nabla f(\x_t), \u_t - \E\u_t\right\rangle = (1-\alpha)^t\E\left\langle \nabla f(\x_{0}), \u_{0} - \m_{0}\right\rangle+ \sum_{s=1}^t(1-\alpha)^{t-s}c_s.
\end{align*}
Since $\A(\x_0;\xi_0) = \nabla F(\x_0;\xi_0)$, which means $\mathbb E_{\xi_0}\b_t = \nabla f(\x_0)$ so that $\E\left\langle \nabla f(\x_{0}), \u_{0} - \m_{0}\right\rangle = 0$. So the equation above becomes 
\begin{align*}
\E\left\langle \nabla f(\x_t), \u_t - \m_t\right\rangle =\sum_{s=1}^t(1-\alpha)^{t-s}c_s,
\end{align*}
and \begin{align*}
\sum_{t=1}^T\E\left\langle \nabla f(\x_t), \u_t - \E\u_t\right\rangle\leq &\frac{\sum_{t=1}^T |c_t|}{1-(1-\alpha)}\\
\leq & \frac{\gamma L}{\alpha}\sum_{t=0}^T\E\|\m_t\|^2 + \frac{3\gamma L}{\alpha}\sum_{t=0}^T\E\|\u_t -\m_t\|^2
.\numberthis\label{lemma:momentum_eq4}
\end{align*}
% In order to upper bound $c_s$, we have
% \begin{align*}
% c_s =& \E\left\langle \nabla f(\x_s) - \nabla f(\x_{s-1}), \u_s - \E\u_s \right\rangle\\
% \leq & \frac{\sqrt{\alpha}}{\gamma}\E\left\|\nabla f(\x_s) - \nabla f(\x_{s-1})\right\|^2 + \frac{\gamma}{\sqrt{\alpha}}\E\left\| \u_s - \E\u_s \right\|^2\\
% \leq & \frac{L^2\sqrt{\alpha}\E\left\|\x_s - \x_{s-1}\right\|^2}{\gamma} + \frac{\gamma}{\sqrt{\alpha}}\E\left\| \u_s - \E\u_s \right\|^2.\numberthis\label{lemma:bound_var_ct_2}
% \end{align*}
For $\E\left\| \u_t - \m_t \right\|^2$, we have
\begin{align*}
\E\|\u_t - \m_t \|^2 = & \E\|(1-\alpha)(\u_{t-1} - \m_{t-1}) + \alpha(\g_t - \nabla f(\x_t)  ) \|^2\\
= & \E_{1:t-1}\E_t\|(1-\alpha)(\u_{t-1} - \m_{t-1}) + \alpha(\g_t - \nabla f(\x_t)  ) \|^2\\
= & \E_{1:t-1}\E_t\|(1-\alpha)(\u_{t-1} - \m_{t-1})\|^2 + \E_{1:t-1}\E_t\|\alpha(\g_t - \nabla f(\x_t)  ) \|^2\\
= & (1-\alpha)^2\E\|\u_{t-1} - \m_{t-1}\|^2 + \alpha^2\sigma^2.
\end{align*}
Therefore we have
\begin{align*}
\sum_{t=0}^T\E\|\u_t - \m_t \|^2\leq \alpha\sigma^2.
\end{align*}
So \eqref{lemma:momentum_eq4} becomes
\begin{align*}
\sum_{t=1}^T\E\left\langle \nabla f(\x_t), \u_t - \E\u_t\right\rangle\leq \frac{\gamma L}{\alpha}\sum_{t=0}^T\E\|\m_t\|^2 + 2\gamma L\sigma^2.\numberthis\label{lemma:momentum_eq5}
\end{align*}
Combing \eqref{lemma:momentum_eq0} with \eqref{lemma:momentum_eq1} and \eqref{lemma:momentum_eq5}, we have
\begin{align*}
&\E\|\nabla f(\x_t) - \u_{t}\|^2 - \E\|\u_{t}\|^2\\
\leq & -\left(1 - \frac{L^2\gamma^2}{\alpha^2} - \frac{\gamma L}{\alpha}  \right)\E\|\m_t\|^2 + 2\gamma L\sigma^2.
\end{align*}
Therefore for \textbf{Momentum SGD},
\begin{align*}
A_t = &  \E\|\nabla f({\x}_t) - {\u}_{t}\|^2 - (1-2L\gamma)\E\|{\u}_{t}\|^2 - \frac{1}{4}\E\|\nabla f(\x_t)\|^2\\
\leq & -\left(1 - \frac{L^2\gamma^2}{\alpha^2} - \frac{\gamma L}{\alpha}  \right)\E\|\m_t\|^2 + 2\gamma L\sigma^2 + 2L\gamma\E\|{\u}_{t}\|^2\\
\leq & -\left(1 - \frac{L^2\gamma^2}{\alpha^2} - \frac{\gamma L}{\alpha}  \right)\E\|\m_t\|^2 + 2\gamma L\sigma^2 + 4L\gamma\E\|{\m}_{t}\|^2 + 4L\gamma \alpha\sigma^2\\
= & -\left(1 - 4L\gamma - \frac{L^2\gamma^2}{\alpha^2} - \frac{\gamma L}{\alpha}  \right)\E\|\m_t\|^2 + 6\gamma L\sigma^2 .
\end{align*}
So if $L\gamma\leq \frac{\alpha}{8}$, we have
\begin{align*}
\sum_{t=0}^TA_t \leq 6\gamma L\sigma^2T
\end{align*}

\end{proof}
% Therefore we have
% \begin{align*}
% &\sum_{s=1}^t(1-\alpha)^{t-s}\E\|\u_s - \E\u_s \|^2\\
% =& \sum_{s=1}^t(1-\alpha)^{t-s}\left((1-\alpha)^{2s}\E\|\u_{0} - \hu_{0}\|^2 + \alpha^2\sum_{r=1}^s(1-\alpha)^{2(s-r)}\alpha^2\E\|\b_r - \E_r\b_r\|^2\right)\\
% = &\sum_{s=1}^t(1-\alpha)^{t+s}\E\|\u_{0} - \hu_{0}\|^2 + \alpha^2\sum_{s=1}^t\sum_{r=1}^s(1-\alpha)^{t-s+2s-2r}\E\|\b_r - \E_r\b_r\|^2\\
% = & \sum_{s=1}^t(1-\alpha)^{t+s}\E\|\u_{0} - \hu_{0}\|^2 + \alpha^2\sum_{r=1}^t(1-\alpha)^{t-2r}\E\|\b_r - \E_r\b_r\|^2\left(\sum_{s=r}^t(1-\alpha)^{s}\right)\\
% \end{align*}

% \begin{align*}
% &\sum_{t=1}^T\sum_{s=1}^t\sum_{r=1}^s\rho^{t-s}\rho^{2(s-r)}b_r\\
% = & \sum_{t=1}^T\sum_{r=1}^t\rho^{t-2r}b_r\left(\sum_{s=r}^t\rho^{s}\right)\\
% = & \sum_{t=1}^T\sum_{r=1}^t\frac{\rho^{t-2r}(\rho^{r} - \rho^{t+1})}{1-\rho}b_r\\
% = & \sum_{t=1}^T\sum_{r=1}^t\frac{\rho^{t-r} - \rho^{2t-2r+1}}{1-\rho}b_r\\
% = & \sum_{s=1}^T\frac{b_r}{1-\rho}\left(\sum_{t=r}^T\rho^{t-r} -\sum_{t=r}^T \rho^{2t-2r+1}\right)\\
% = & \sum_{s=1}^T\frac{b_r}{1-\rho}\left(\frac{1-\rho^{T-r+1}}{1-\rho} -\frac{\rho - \rho^{2T - 2r +3} }{1-\rho^2}\right)\\
% = & \sum_{s=1}^T\frac{b_r}{1-\rho}\left(\frac{1-\rho^2 - \rho^{T-r+1}(1-\rho^2) - \rho(1- \rho) + \rho^{2T - 2r+3}(1-\rho)   }{(1-\rho)(1-\rho^2)} \right)\\
% = & \sum_{s=1}^T\frac{b_r}{1-\rho}\left(\frac{1-\rho - (1-\rho^2)\rho^{T-r+1} + \rho^{2T - 2r+3}(1-\rho)  }{(1-\rho)(1-\rho^2)} \right)\\
% = & \sum_{s=1}^T\frac{b_r}{1-\rho}\left(\frac{1 - (1+\rho)\rho^{T-r+1} + \rho^{2T - 2r+3}  }{1-\rho^2} \right)\\
% \end{align*}


% \newpage
% Therefore from Lemma~\ref{lemma:contraction}, we have
% \begin{align*}
% \sum_{t=0}^T\E\|\u_t - \hu_t \|^2 \leq & \frac{\E\|\u_0 - \hu_0 \|^2 +\alpha^2\sum_{t=1}^T\E\|\b_t - \E_t\b_t\|^2}{1- (1-\alpha)^2}\\
% \leq & \frac{\sigma^2 }{B_0\alpha} +\alpha\sum_{t=1}^T\E\|\b_t - \E_t\b_t\|^2
% .\numberthis\label{lemma:bound_var_ct_3}
% \end{align*}
% Combining \eqref{lemma:bound_var_ct_1}, \eqref{lemma:bound_var_ct_2} and \eqref{lemma:bound_var_ct_3} together we get
% \begin{align*}
% &\sum_{t=1}^T\E\left\langle \nabla f(\x_t), \u_t - \hu_t\right\rangle\\
% \leq & \frac{L^2\E\left\|\x_t - \x_{t-1}\right\|^2}{\gamma\sqrt{\alpha}} + \frac{\sigma^2 }{B_0\alpha} +\alpha\sum_{t=1}^T\E\|\b_t - \E_t\b_t\|^2
% \end{align*}
% 




% \newpage
% \begin{lemma}\label{lemma:general_step2}
% For any gradient estimator that is constructed following \eqref{update:u_t}, we have
% \begin{align*}
% &\sum_{t=1}^{T}\mathbb{E}\|\mathbb E_t\u_t - \nabla f(\x_t)\|^2\\
% \leq & \frac{\alpha\sigma^2}{B_0} + 6\Delta_b^{\mathscr{A}}T + 3\alpha(1-\alpha)^2\Delta_v^{\mathscr{A}}T+ 4\sum_{t=0}^{T-1}\left( \mathbb{E} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] +2\alpha(1-\alpha)^2\mathbb{E} \left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]\right).
% \end{align*}
% \end{lemma}
% % =& \mathbb{E}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_t\b_t - \nabla f(\x_t) + (1-\alpha)\nabla f(\x_t) + (1-\alpha)(\u_{t-1} - \mathbb E_{t-1}\u_{t-1})  \right\|^2\\
% % =& \mathbb{E}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t + (1-\alpha)(\u_{t-1} - \mathbb E_{t-1}\u_{t-1}) \right\|^2\\
% % =& \mathbb{E}_{1:t-2}\mathbb E_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t + (1-\alpha)(\u_{t-1} - \mathbb E_{t-1}\u_{t-1})  \right\|^2\\
% % =& \mathbb{E}_{1:t-2}\mathbb E_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t \right\|^2+ (1-\alpha)^2\mathbb{E}_{1:t-2}\mathbb E_{t-1}\left\|\u_{t-1} - \mathbb E_{t-1}\u_{t-1}   \right\|^2\\
% % =& \mathbb{E}_{1:t-2}\mathbb E_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_{t-1}\z_t + \alpha(\z_t - \mathbb E_{t-1}\z_t) \right\|^2+ \alpha^2(1-\alpha)^2\mathbb{E}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}   \right\|^2\\
% % =& \mathbb{E}_{1:t-2}\mathbb E_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_{t-1}\z_t\right\|^2 + \alpha^2\mathbb E\left\|\z_t - \mathbb E_{t-1}\z_t \right\|^2+ \alpha^2(1-\alpha)^2\mathbb{E}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}   \right\|^2\\
% % =& \mathbb{E}_{1:t-2}\left(\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_{t}\z_t  \right\|^2 + \alpha^2\mathbb E_{t}\|\z_t - \mathbb E_{t}\z_t\|^2 \right)\\
% \begin{proof}
% Denote $\b_t := \mathscr{A}(\x_t;\xi_t)$, $\e_t :=  \mathbb E_t\u_t - \nabla f(\x_t)$ and $\z_t = \mathbb E_t\b_t - \frac{\nabla f(\x_t) - (1-\alpha)\nabla f(\x_{t-1})}{\alpha}$,  we get
% \begin{align*}
% \mathbb E_t\u_t = (1-\alpha)\u_t + \alpha\mathbb E_t\b_t,
% \end{align*}
% which leads to
% \begin{align*}
% &\mathbb{E}_{t-1}\|\e_t\|^2\\
% =& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_t\b_t - \nabla f(\x_t) + (1-\alpha)\nabla f(\x_t) + (1-\alpha)(\u_{t-1} - \mathbb E_{t-1}\u_{t-1})  \right\|^2\\
% =& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_t\b_t - \nabla f(\x_t) + (1-\alpha)\nabla f(\x_t) + \alpha(1-\alpha)(\b_{t-1} - \mathbb E_{t-1}\b_{t-1})  \right\|^2\\
% =& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t + \alpha(1-\alpha)(\b_{t-1} - \mathbb E_{t-1}\b_{t-1})  \right\|^2\\
% =& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t\right\|^2 + (1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2\\
% &+ 2\mathbb E_{t-1}\left\langle\e_{t-1} + \alpha\z_t,(1-\alpha)\alpha(\b_{t-1} - \mathbb E_{t-1}\b_{t-1}) \right\rangle \\
% =& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t\right\| + (1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2+ 2\alpha^2\mathbb E_{t-1}\left\langle  \z_t,(1-\alpha)(\b_{t-1} - \mathbb E_{t-1}\b_{t-1}) \right\rangle \\
% \leq& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t\right\|^2 + (1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2\\
% &+ 2\alpha^2\mathbb E_{t-1}\left\| \z_t\right\|^2 + 2\alpha^2(1-\alpha)^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1} \right\|^2 \\
% \leq& \mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1} + \alpha\z_t\right\|^2 + 3(1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2+ 2\alpha^2\mathbb E_{t-1}\left\| \z_t\right\|^2  \\
% \leq& (1+\alpha)\mathbb{E}_{t-1}\left\|(1-\alpha)\e_{t-1}\right\|^2 + \left( 1+ \frac{1}{\alpha}\right)\mathbb E_{t-1}\left\|\alpha\z_t\right\|^2 + 3(1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2+ 2\alpha^2\mathbb E_{t-1}\left\| \z_t\right\|^2  \\
% \leq& (1-\alpha)\mathbb{E}_{t-1}\left\|\e_{t-1}\right\|^2 + 4\alpha\mathbb E_{t-1}\left\|\z_t\right\|^2 + 3(1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2  \\
% \leq& (1-\alpha)\left\|\e_{t-1}\right\|^2 + 4\alpha\mathbb E_{t-1}\left\|\mathbb E_{t}\b_t - \frac{\nabla f(\x_t) - (1-\alpha)\nabla f(\x_t)}{\alpha}\right\|^2 + 3(1-\alpha)^2\alpha^2\mathbb E_{t-1}\left\|\b_{t-1} - \mathbb E_{t-1}\b_{t-1}  \right\|^2  \\
% \leq & \left(1-\alpha\right)\left\|\e_{t-1}\right\|^2 + 4\alpha\Delta_b^\A + 3\alpha^2(1-\alpha)^2\Delta_v^\A\\
% &+ 4\alpha \mathbb{E}_{t-1} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] + 3\alpha^2(1-\alpha)^2\mathbb E_{t-1}\left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]
% \end{align*}
% % Denote $\b_t := \mathscr{A}(\x_t;\xi_t)$, $\e_t :=  \u_t - \nabla f(\x_t)$ and $\z_t = \b_t - \frac{\nabla f(\x_t) - (1-\alpha)\nabla f(\x_{t-1})}{\alpha}$,  we get
% % \begin{align*}
% % \mathbb{E}\|\e_t\|^2 = &\mathbb{E}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_t\b_t - \nabla f(\x_t) + (1-\alpha)\nabla f(\x_t) + \alpha(\b_t - \mathbb E_t \b_t)  \right\|^2\\
% % =& \mathbb{E}_{1:t-1}\left(\mathbb E_t\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_{t}\z_t  \right\|^2 + \alpha^2\mathbb E_{t}\|\b_t - \mathbb E_{t}\b_t\|^2 \right)\\
% % =& \mathbb{E}\left\|(1-\alpha)\e_{t-1} + \alpha\mathbb E_{t}\z_t  \right\|^2 + \alpha^2\mathbb E\|\b_t - \mathbb E_{t}\b_t\|^2 \\
% % \leq& \mathbb{E}\left(\left((1-\alpha)^2 + \alpha\right)\left\|\e_{t-1}\right\|^2 +\left(1 + \frac{1}{\alpha}\right) \|\alpha\mathbb E_{t}\z_t  \|^2\right) + \alpha^2\mathbb E\|\b_t - \mathbb E_{t}\b_t\|^2 \\
% % \leq& \left(1-\alpha\right)\mathbb{E}\left\|\e_{t-1}\right\|^2 + 2\alpha\mathbb{E} \|\mathbb E_{t}\z_t  \|^2 + \alpha^2\mathbb E\|\b_t - \mathbb E_{t}\b_t\|^2\\
% % =&\mathbb{E}\left(1-\alpha\right)\mathbb{E}\left\|\e_{t-1}\right\|^2 + 2\alpha\mathbb{E} \left\|\mathbb E_{t}\b_t - \frac{\nabla f(\x_t) - (1-\alpha)\nabla f(\x_t)}{\alpha} \right\|^2 + \alpha^2\mathbb E\|\b_t - \mathbb E_{t}\b_t\|^2\\
% % \leq & \mathbb{E}\left(1-\alpha\right)\mathbb{E}\left|\e_{t-1}\right\|^2 + 2\alpha \mathbb{E} \left[ \Delta_b^{\mathscr{A}} +  M_{b}^\A(\|\x_{t} - \x_{t-1}\|)  \right] + \alpha^2\mathbb E\left[ \Delta_v^{\mathscr{A}} +  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]\\
% % \leq & \mathbb{E}\left(1-\alpha\right)\mathbb{E}\left|\e_{t-1}\right\|^2 + 2\alpha\Delta_b^\A + \alpha^2\Delta_v^\A + 2\alpha \mathbb{E} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] + \alpha^2\mathbb E\left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]
% % \end{align*}
% Taking the expectation over all history information, combined with Lemma~\ref{lemma:contraction}, we get 
% \begin{align*}
% &\sum_{t=1}^{T}\mathbb{E}\|\e_t\|^2\\
% \leq & \frac{\sum_{t=1}^{T}\left(4\alpha\Delta_b^\A + 3\alpha^2(1-\alpha)^2\Delta_v^\A + 4\alpha \mathbb{E} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] + 3\alpha^2(1-\alpha)^2\mathbb E\left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]  \right) + \mathbb{E}\|\e_1\|^2}{1- (1-\alpha)}\\
% \leq & \frac{\mathbb E\|\e_1\|^2}{\alpha} + 4\Delta_b^{\mathscr{A}}T + 3\alpha(1-\alpha)^2\Delta_v^{\mathscr{A}}T + 2\sum_{t=0}^{T-1}\left( \mathbb{E} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] +2\alpha(1-\alpha)^2\mathbb{E} \left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]\right).\numberthis\label{theo:general_et_eq1}
% \end{align*}
% Notice that we have $\e_0 = \bm{0}$ because $\A(\x_0;\xi_0) = \nabla F(\x_t;\xi_t)$, therefore or $\e_1$ we have
% \begin{align*}
% \mathbb{E}_{0}\|\e_1\|^2
% =& \mathbb{E}_{0}\left\|\alpha\mathbb E_1\b_1 - \nabla f(\x_1) + (1-\alpha)\nabla f(\x_0) + (1-\alpha)(\nabla F(\x_t;\xi_t) - \nabla f(\x_t))  \right\|^2\\
% =& \mathbb{E}_{0}\left\|\alpha\z_1 + (1-\alpha)(\nabla F(\x_t;\xi_t) - \nabla f(\x_t))  \right\|^2\\
% \leq & 2\alpha^2\left(\Delta_b^\A + M_b^\A(\|\x_1 - \x_0\|)  \right) + 2(1-\alpha)^2\frac{\sigma^2}{B_0}.\numberthis\label{theo:general_et_eq2}
% \end{align*}
% Combining \eqref{theo:general_et_eq1} and \eqref{theo:general_et_eq2} together we get
% \begin{align*}
% \sum_{t=1}^{T}\mathbb{E}\|\e_t\|^2
% \leq & \frac{(1-\alpha)^2\sigma^2}{\alpha B_0} + 6\Delta_b^{\mathscr{A}}T + 3\alpha(1-\alpha)^2\Delta_v^{\mathscr{A}}T\\
% &+ 4\sum_{t=0}^{T-1}\left( \mathbb{E} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] +2\alpha(1-\alpha)^2\mathbb{E} \left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]\right).
% \end{align*}

% \end{proof}

% \section{Proof of Theorem~\ref{theo:general}}
% \begin{proof}
% According to Lemma~\ref{lemma:general_step1}, we have
% \begin{align*}
% &\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2 + \frac{1 }{2 T}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbb E_t\u_t\|^2 \\
% \leq & \frac{2(f(\x_{0}) - f^*)}{\gamma T}  + \frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t) - \mathbb E_t\u_t\|^2 + \frac{8L^2}{T}\sum_{t=0}^{T-1}\mathbb E\|\hat{\x}_t - \x_t\|^2 + \frac{\gamma}{T}\sum_{t=1}^{T-1}\mathbb E\|\u_t\|^2.
% \end{align*}
% Then using Lemma~\ref{lemma:general_step2} for upper bounding $\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t) -\mathbb E_t \u_t\|^2$, we get
% \begin{align*}
% &\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2 + \frac{1 }{2 T}\sum_{t=0}^{T-1}\mathbb{E}\|\mathbb E_t\u_t\|^2 \\
% \leq & \frac{2(f(\x_{0}) - f^*)}{\gamma T}   + \frac{8L^2}{T}\sum_{t=0}^{T-1}\mathbb E\|\hat{\x}_t - \x_t\|^2 + \frac{\gamma}{T}\sum_{t=1}^{T-1}\mathbb E\|\u_t\|^2+ \frac{(1-\alpha)^2\sigma^2}{\alpha B_0 T} + 6\Delta_b^{\mathscr{A}} + 3\alpha(1-\alpha)^2\Delta_v^{\mathscr{A}}\\
% &+ \frac{4}{T}\sum_{t=0}^{T-1}\left( \mathbb{E} \left[  M_{b}^\A(\|\x_t - \x_{t-1}\|)  \right] +2\alpha(1-\alpha)^2\mathbb{E} \left[  M_{v}^\A(\|\x_t - \x_{t-1}\|)  \right]\right).
% \end{align*}
% Then using Lemma~\ref{lemma:update_different_alg} for upper bounding $\|\hat{\x}_t - \x_t\|$ and $\|\x_t - \x_{t-1}\|$ for each algorithm will finish the proof.
% \end{proof}




\begin{lemma}\label{lemma:bound_et}
For STROM (without compression),  we have the following upper bound for $\sum_{t=0}^{T-1}\mathbb{E}\|\u_t - \nabla f(\x_t)\|^2$:
\begin{align*}
\sum_{t=0}^{T-1} A_t \leq \frac{2\alpha\sigma^2 T}{n}   + \frac{\mathbb{E}\|\u_0 - \nabla f(\x_0)\|^2}{\alpha}.
\end{align*}
\end{lemma}
\begin{proof}
For STROM, the most import part is to upper bound $\sum_{t=0}^{T-1}\mathbb{E}\|\u_t - \nabla f(\x_t)\|^2$.  Therefore we first focus on this term.

Denoting $\e_t := \u_t - \nabla f(\x_t)$ and $\og_t(\x) :=\frac{1}{n}\sum_{i}\nabla F(\x;\xi_t^\bi)$, we get
\begin{align*}
\mathbb{E}\|\e_t\|^2 =& \mathbb{E}\|(1-\alpha)\e_{t-1} + (\og_t(\x_t) -\nabla f(\x_t)) - (1-\alpha)(\og_{t}(\x_{t-1}) - \nabla f(\x_{t-1})) \|^2\\
= & \mathbb{E}\|(1-\alpha)\e_{t-1}\|^2 +\mathbb{E}\| (\og_t(\x_t) -\nabla f(\x_t)) - (1-\alpha)(\og_{t}(\x_{t-1}) - \nabla f(\x_{t-1})) \|^2\\
= & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + \mathbb{E}\left\|\alpha(\og_t(\x_t) -\nabla f(\x_t)) + (1-\alpha)\left(\og_t(\x_t) - \og_t(\x_{t-1}) + \nabla f(\x_{t-1}) - \nabla f(\x_t)  \right)   \right\|^2 \\
\leq & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + 2\alpha^2\mathbb{E}\left\|\og_t(\x_t) -\nabla f(\x_t)\right\|^2 + 2(1-\alpha)^2\mathbb{E}\left\|\og_t(\x_t) - \og_t(\x_{t-1}) + \nabla f(\x_{t-1}) - \nabla f(\x_t)    \right\|^2 \\
= & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + 2\alpha^2\mathbb{E}\left\|\og_t(\x_t) -\nabla f(\x_t)\right\|^2\\
&+ \frac{2(1-\alpha)^2}{n^2}\mathbb{E}\left\|\sum_{i=1}^n\left(\nabla F(\x_t;\xi_t^\bi) - \nabla f_i(\x_t) - \nabla F(\x_{t-1};\xi_{t-1}^\bi) + \nabla f_i(\x_{t-1}) \right)    \right\|^2 \\
= & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + 2\alpha^2\mathbb{E}\left\|\og_t(\x_t) -\nabla f(\x_t)\right\|^2\\
&+ \frac{2(1-\alpha)^2}{n^2}\sum_{i=1}^n\mathbb{E}\left\|\nabla F(\x_t;\xi_t^\bi) - \nabla f_i(\x_t) - \nabla F(\x_{t-1};\xi_{t-1}^\bi) + \nabla f_i(\x_{t-1})    \right\|^2 \\
\leq & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + 2\alpha^2\mathbb{E}\left\|\og_t(\x_t) -\nabla f(\x_t)\right\|^2\\
&+ \frac{2(1-\alpha)^2}{n^2}\sum_{i=1}^n\mathbb{E}\left\|\nabla F(\x_t;\xi_t^\bi)  - \nabla F(\x_{t-1};\xi_{t-1}^\bi)    \right\|^2 \\
\leq & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + \frac{2\alpha^2\sigma^2}{n} + \frac{2(1-\alpha)^2L^2}{n}\mathbb{E} \|\x_t - \x_{t-1}\|^2\\
\leq & (1-\alpha)^2 \mathbb{E}\|\e_{t-1}\|^2 + \frac{2\alpha^2\sigma^2}{n} + \frac{2(1-\alpha)^2L^2\gamma^2}{n}\mathbb{E} \|\v_{t-1}\|^2.\numberthis\label{proof:storm_bound_et}
\end{align*}
Using Lemma~\ref{lemma:contraction}, we get 
\begin{align*}
\sum_{t=0}^{T-1}\mathbb{E}\|\e_t\|^2 \leq & \frac{\sum_{t=0}^{T-1}\left( \frac{2\alpha^2\sigma^2}{n} + \frac{2(1-\alpha)^2L^2\gamma^2}{n}\mathbb{E} \|\v_{t-1}\|^2 \right) + \mathbb{E}\|\e_0\|^2}{1- (1-\alpha)^2}\\
\leq & \frac{1}{\alpha}\left( \frac{2\alpha^2\sigma^2 T}{n} + \frac{2(1-\alpha)^2L^2\gamma^2}{n}\sum_{t=0}^{T-1}\mathbb{E} \|\v_{t-1}\|^2 + \mathbb{E}\|\e_0\|^2 \right)\\
\leq & \frac{1}{\alpha}\left( \frac{2\alpha^2\sigma^2 T}{n} + \frac{2(1-\alpha)^2L^2\gamma^2}{n}\sum_{t=0}^{T-1}\mathbb{E} \|\v_{t-1}\|^2 + \mathbb{E}\|\e_0\|^2 \right).\numberthis\label{theo:storm_eq1}
\end{align*}
It can be easily verified that when $\beta = 1$, we have
\begin{align*}
\v_t = \u_t - \alpha\odelta_t + \alpha\odelta_{t-1}.\numberthis\label{theo:storm_vt_ut}
\end{align*}
Combing \eqref{theo:storm_eq1} and \eqref{theo:storm_vt_ut} we get
\begin{align*}
\sum_{t=0}^{T-1}\mathbb{E}\|\e_t\|^2 \leq &  \frac{1}{\alpha}\left( \frac{2\alpha^2\sigma^2 T}{n} + \frac{2(1-\alpha)^2L^2\gamma^2}{n}\sum_{t=0}^{T-1}\mathbb{E} \|\u_{t-1} - \alpha\bdelta_{t-1} + \alpha\bdelta_{t-2}\|^2 + \mathbb{E}\|\e_0\|^2 \right)\\
\leq & \frac{1}{\alpha}\left( \frac{2\alpha\sigma^2 T}{n} + \frac{4(1-\alpha)^2L^2\gamma^2}{n}\sum_{t=0}^{T-1}\left(\mathbb{E} \|\u_{t-1}\|^2 + 2\alpha^2\mathbb E\|\bdelta_{t-1}\|^2\right)  + \mathbb{E}\|\e_0\|^2 \right)\\
\leq & \frac{2\alpha^2\sigma^2 T}{n} + \frac{4(1-\alpha)^2L^2\gamma^2}{\alpha n} \sum_{t=0}^{T-1}\mathbb{E} \|\u_{t-1}\|^2 + \frac{4(1-\alpha)^2L^2\alpha\gamma^2\epsilon^2T}{n} + \frac{\mathbb{E}\|\e_0\|^2}{\alpha}.
\end{align*}
Therefore if $\frac{4(1-\alpha)^2L^2\gamma^2}{\alpha n} \leq \frac{1}{2}$ and $1-L\gamma\geq \frac{1}{2}$, then we have
\begin{align*}
\sum_{t=0}^{T-1} A_t \leq \frac{2\alpha\sigma^2 T}{n}  + \frac{4(1-\alpha)^2L^2\alpha\gamma^2\epsilon^2T}{n} + \frac{\mathbb{E}\|\u_0 - \nabla f(\x_0)\|^2}{\alpha}.
\end{align*}

\end{proof}


\begin{lemma}\label{lemma:bound_et_strongly}
For STROM (without compression),  we have the following upper bound for $\sum_{t=0}^{T-1}\mathbb{E}\|\u_t - \nabla f(\x_t)\|^2$:
\begin{align*}
\sum_{t=0}^{T-1} A_t \leq \frac{2\alpha\sigma^2 T}{n}   + \frac{\mathbb{E}\|\u_0 - \nabla f(\x_0)\|^2}{\alpha}.
\end{align*}
\end{lemma}

\begin{proof}
From \eqref{proof:storm_bound_et}, we have
\begin{align*}
&\E\|\nabla f(\x_t) - \u_t\|^2 - \E\|\nabla f(\x_t)\|^2\\
\leq &  (1-\alpha_t) \mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 + \frac{2\alpha_t^2\sigma^2}{n} + \frac{2(1-\alpha_t)^2L^2\gamma_t^2}{n}\mathbb{E} \|\u_{t-1}\|^2- \E\|\nabla f(\x_t)\|^2\\
= & (1-\alpha_t) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}\\
&+ \frac{2(1-\alpha_t)^2L^2\gamma_t^2}{n}\mathbb{E} \|\u_{t-1}\|^2- \E\|\nabla f(\x_t)\|^2 + (1-\alpha_t)\E\|\nabla f(\x_{t-1})\|^2\\
= & (1-\alpha_t) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}\\
&+ \frac{2(1-\alpha_t)^2L^2\gamma_t^2}{n}\mathbb{E} \|\u_{t-1}\|^2- \left(\E\|\nabla f(\x_t)\|^2 - \E\|\nabla f(\x_{t-1})\|^2\right) -\alpha_t\E\|\nabla f(\x_{t-1})\|^2\\
\leq & (1-\alpha_t) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}\\
&+ \frac{2(1-\alpha_t)^2L^2\gamma_t^2}{n}\mathbb{E} \|\u_{t-1}\|^2 +  \gamma_t^2L^2\E\|\u_{t-1}\|^2 -\alpha_t\E\|\nabla f(\x_{t-1})\|^2\\
\leq & (1-\alpha_t) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}\\
&+ \frac{2L^2\gamma_t^2}{n}\mathbb{E} \|\u_{t-1}\|^2 +  \gamma_t^2L^2\E\|\u_{t-1}\|^2 -\alpha_t\E\|\nabla f(\x_{t-1})\|^2\\
\leq & (1-\alpha_t) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}\\
& +  3\gamma_t^2L^2\E\|\u_{t-1}\|^2 -\alpha_t\E\|\nabla f(\x_{t-1})\|^2\\
\leq & (1-\alpha_t) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}\\
& +  6\gamma_t^2L^2\E\|\nabla f(\x_{t-1})\|^2 + 6\gamma_t^2L^2\E \|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 -\alpha_t\E\|\nabla f(\x_{t-1})\|^2\\
= & (1-\alpha_t + 6\gamma^2_tL^2) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}  -(\alpha_t-6\gamma_t^2L^2)\E\|\nabla f(\x_{t-1})\|^2.
\end{align*}
Now that if $\alpha_t \geq 12\gamma_t^2L^2$, we would have
\begin{align*}
&\E\|\nabla f(\x_t) - \u_t\|^2 - \E\|\nabla f(\x_t)\|^2
\leq & \left(1-\frac{\alpha_t}{2} \right) \left(\mathbb{E}\|\nabla f(\x_{t-1}) - \u_{t-1}\|^2 - \E\|\nabla f(\x_{t-1})\|^2 \right) + \frac{2\alpha_t^2\sigma^2}{n}.
\end{align*}
\end{proof}


\section{Proof to Corollary}
From Theorem~\ref{theo:main}, we have
\begin{align*}
\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2\leq 
\frac{2( f(\x_{0}) -  f^*)}{\gamma T} + \frac{4\alpha\sigma^2 (1 + 8nL^2\gamma^2D_{\omega})}{n} +32\alpha L^2\gamma^2D_{\omega}\zeta^2   + \frac{\sigma^2}{n\alpha T S_0}.
\end{align*}
By setting $\gamma = \frac{n^{\frac{2}{3}}}{(\sigma^2 T)^\frac{1}{3}L + (\zeta^2 T)^{\frac{1}{5}} + 4L}$, $\alpha = \frac{128n^{\frac{1}{3}}}{(\sigma^2 T)^{\frac{2}{3}}  + (\zeta^2 T)^{\frac{2}{5}} + 8 }$ and $S_0 = \frac{ (\sigma^2T)^\frac{1}{3}}{n^{\frac{2}{3}}}$, we can guarantee that $\gamma\leq  \frac{1}{4L}$ and $ 128L^2\gamma^2\leq \alpha\leq \frac{1}{8}$.
Moreover, if  $T\geq\max\left\{\frac{D_{\omega}^{1.5}}{\sigma^2 n^2},\frac{1500D_{\omega}^{0.75}}{\sigma^2 n^{0.5}}  \right\}$, then we  would get $L^2\gamma^2\leq\frac{1}{D_\omega}$ and $\alpha^2\leq\frac{1}{D_\omega}$. In this case, all restrictions for Theorem~\ref{theo:main} are satisfied.
% Therefore we get the final rate
% \begin{align*}
% \frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2\leq &
% 2( f(\x_{0}) -  f^*)\left(\frac{\sigma^{\frac{2}{3}} L}{n^{\frac{2}{3}}T^\frac{2}{3}} + \frac{4L}{n^{\frac{2}{3}}T}\right) + \frac{4\sigma^{\frac{2}{3}} }{n^{\frac{2}{3}}T^{\frac{2}{3}}}\left(1 + \frac{8n^{\frac{7}{3}}D_{\omega}}{\sigma^{\frac{2}{3}}T^{\frac{2}{3}}+ 16  }\right)\\
% &+ \frac{32n^{\frac{5}{3}} D_{\omega}\zeta^2}{\sigma^{\frac{4}{3}}T^\frac{4}{3} + 32}   + \frac{\sigma^{\frac{10}{3}}}{n^{\frac{2}{3}} T^{\frac{2}{3}} }.
% \end{align*}

Treating $( f(\x_{0}) -  f^*)$, $L$ as constants, we get
\begin{align*}
\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\|\nabla f(\x_t)\|^2\lesssim 
\sigma^{\frac{2}{3}}\left( \frac{1 + \sigma^2}{(nT)^{\frac{2}{3}}} + \frac{D_\omega n^{\frac{5}{3}}}{\sigma^{\frac{2}{3}}T^{\frac{4}{3}} + (nT)^{\frac{2}{3}}}  \right) + \frac{n^{\frac{5}{3}} D_{\omega}\zeta^2}{\zeta^{\frac{4}{5}} T^\frac{4}{5} + \sigma^2T^{\frac{4}{3}} } + \frac{1}{T}.
\end{align*}


% whereas for $\Delta_t$, we have
% \begin{align*}
% \v_t =& \v_{t-1} + C_{\omega}\left[\Delta_t\right]\\
% = & \v_{t-1} - \bdelta_{t} + \Delta_t.
% \end{align*}
% So we get
% \begin{align*}
% \Delta_t =& \v_t - \v_{t-1} + \bdelta_t\\
% =& -\alpha\v_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1}) + (2-\alpha) \odelta_{t-1} - (1-\alpha)\odelta_{t-2}-\odelta_t + \bdelta_t\\
% = & -\alpha(\u_{t-1} - \odelta_{t-1} + \odelta_{t-2}) + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1}) + (2-\alpha) \odelta_{t-1} - (1-\alpha)\odelta_{t-2}-\odelta_t + \bdelta_t\\
% =& -\alpha\u_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1})  + 2 \odelta_{t-1} - \odelta_{t-2}-\odelta_t + \bdelta_t\\
% = & -\alpha\u_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1})  + 2 \odelta_{t-1} - \odelta_{t-2}-\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi.
% \end{align*}
% Therefore we get
% \begin{align*}
% &\mathbb{E}\|\Delta_t\|^2\\
% \leq &  \mathbb{E}\left\|  -\alpha\u_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1})  + 2 \odelta_{t-1} - \odelta_{t-2}-\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi    \right\|^2\\
% \leq &  (1+10)\mathbb{E}\left\|  -\alpha\u_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1})\right\|^2  +\frac{11}{10}\mathbb{E}\left\| 2 \odelta_{t-1} - \odelta_{t-2}-\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi    \right\|^2\\
% \leq &  (1+10)\mathbb{E}\left\|  -\alpha\u_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1})\right\|^2  +\frac{11}{10}\left(2\mathbb{E}\left\| 2 \odelta_{t-1} - \odelta_{t-2}\right\|^2 + 2\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi    \right\|^2\right)\\
% \leq & 11 \mathbb{E}\left\|  -\alpha\u_{t-1} + \og_t(\x_t) - (1-\alpha)\og_t(\x_{t-1})\right\|^2  +11\left(\mathbb{E}\left\|  \odelta_{t-1}\right\|^2 + \mathbb{E}\left\| \odelta_{t-2}\right\|^2 \right) + 3\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi    \right\|^2\\
% =& 11 \mathbb{E}\left\|  -\alpha(\u_{t-1}-\og_{t}(\x_{t-1})) + (\og_t(\x_t) - \og_t(\x_{t-1}))\right\|^2  +11\mathbb{E}\left\|  \odelta_{t-1}\right\|^2 + 11\mathbb{E}\left\| \odelta_{t-2}\right\|^2 + 3\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi    \right\|^2.\numberthis\label{bound_Delta:1}
% \end{align*}
% Here $\mathbb{E}\left\|  -\alpha(\u_{t-1}-\og_{t}(\x_{t-1})) + (\og_t(\x_t) - \og_t(\x_{t-1}))\right\|^2$ can be upper bounded according to:
% \begin{align*}
% &\mathbb{E}\left\|  -\alpha(\u_{t-1}-\og_{t}(\x_{t-1})) + (\og_t(\x_t) - \og_t(\x_{t-1}))\right\|^2\\
% \leq & \alpha^2 \mathbb{E}\left\|\u_{t-1}-\og_{t}(\x_{t-1})\right\|^2 + 2\mathbb{E}\left\|\og_t(\x_t) - \og_t(\x_{t-1})\right\|^2  \\
% \leq & \alpha^2 \mathbb{E}\left\|\u_{t-1}-\nabla f(\x_{t-1}) + \nabla f(\x_{t-1}) -\og_{t}(\x_{t-1})\right\|^2 + 2\mathbb{E}\left\|\og_t(\x_t) - \og_t(\x_{t-1})\right\|^2\\
% \leq &\alpha^2 \mathbb{E}\left\|\u_{t-1}-\nabla f(\x_{t-1})\right\|^2 + 2\alpha^2 \sigma^2 + 2L^2\gamma^2\mathbb{E}\|\v_{t-1}\|^2+11\mathbb{E}\left\|  \odelta_{t-1}\right\|^2\\
% = &2\alpha^2 \mathbb{E}\left\|\e_{t-1}\right\|^2 + 2\alpha^2 \sigma^2 + 2L^2\gamma^2\mathbb{E}\|\v_{t-1}\|^2.\numberthis\label{bound_Delta:2}
% \end{align*}
% Combing \eqref{bound_Delta:1} and \eqref{bound_Delta:2} we get
% \begin{align*}
% &\mathbb{E}\|\Delta_t\|^2\\
% \leq & 60\alpha^2 \mathbb{E}\left\|\e_{t-1}\right\|^2 + 60\alpha^2 \sigma^2 + 6L^2\gamma^2\mathbb{E}\|\v_{t-1}\|^2 + +11\mathbb{E}\left\|  \odelta_{t-1}\right\|^2 + 11\mathbb{E}\left\| \odelta_{t-2}\right\|^2 + 3\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi    \right\|^2,\numberthis\label{bound_Delta}
% \end{align*}
% which means
% \begin{align*}
% &\mathbb{E}\|\bdelta_t\|^2\\
% \leq & 6\omega^2\alpha^2 \mathbb{E}\left\|\e_{t-1}\right\|^2 + 6\omega^2\alpha^2 \sigma^2 + 6L^2\omega^2\gamma^2\mathbb{E}\|\v_{t-1}\|^2  +11\omega^2\mathbb{E}\left\|  \odelta_{t-1}\right\|^2\\
% &+ 11\omega^2\mathbb{E}\left\| \odelta_{t-2}\right\|^2 + 3\omega^2\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi \right\|^2.
% \end{align*}
% Summing up the equation above and following the analysis of \eqref{bound_Delta_i}, we get
% \begin{align*}
% \sum_{t=0}^{T-1}\mathbb{E}\|\bdelta_t\|^2
% \leq & 6\omega^2\alpha^2 \sum_{t=0}^{T-1}\mathbb{E}\left\|\e_{t-1}\right\|^2 + 6\omega^2\alpha^2 \sigma^2 T + 6L^2\omega^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\|\v_{t-1}\|^2\\
% &  +6\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\|  \odelta_{t}\right\|^2 + 3\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi \right\|^2.\numberthis\label{bound_sum_delta}
% \end{align*}

% Now we have already upper bounded $\mathbb{E}\|\bdelta_t^\bi\|^2$ and $\mathbb{E}\|\bdelta_t\|^2$ according to \eqref{bound_sum_Delta_i} and \eqref{bound_sum_delta}, so we are ready to upper bound $\mathbb{E}\|\odelta_t\|^2$ by
% \begin{align*}
% &\sum_{t=0}^T\mathbb{E}\|\odelta_t\|^2\\
% = & \sum_{t=0}^T\mathbb{E}\left\|\bdelta_t + \frac{1}{n}\sum_{i=1}^n \bdelta_t^{\bi}\right\|^2\\
% \leq & 2\sum_{t=0}^T\mathbb{E}\left\|\bdelta_t\right\|^2 + 2\sum_{t=0}^T\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^{\bi}\right\|^2\\
% \leq & 6\omega^2\alpha^2 \sum_{t=0}^{T-1}\mathbb{E}\left\|\e_{t-1}\right\|^2 + 6\omega^2\alpha^2 \sigma^2 T + 6L^2\omega^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\|\v_{t-1}\|^2  +6\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\|  \odelta_{t}\right\|^2\\
% &+ (2+3\omega^2)\sum_{t=0}^{T-1}\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi \right\|^2\\
% \leq & 6\omega^2\alpha^2 \sum_{t=0}^{T-1}\mathbb{E}\left\|\e_{t-1}\right\|^2 + 6\omega^2\alpha^2 \sigma^2 T + 6L^2\omega^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\|\v_{t-1}\|^2  +6\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\|  \odelta_{t}\right\|^2\\
% &+ 3\sum_{t=0}^{T-1}\mathbb{E}\left\|\frac{1}{n}\sum_{i=1}^n \bdelta_t^\bi \right\|^2\quad\text{(due to $(1-15\omega^2)>0$)}\\
% \leq & 6\omega^2\alpha^2 \sum_{t=0}^{T-1}\mathbb{E}\left\|\e_{t-1}\right\|^2 + 6\omega^2\alpha^2 \sigma^2 T + 6L^2\omega^2\gamma^2\sum_{t=0}^{T-1}\mathbb{E}\|\v_{t-1}\|^2  +6\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\|  \odelta_{t}\right\|^2\\
% & + \frac{18\omega^2L^2\gamma^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + \frac{198\omega^2\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{198\omega^2\alpha^2(\sigma^2 + \zeta^2)}{1-15\omega^2} + \frac{18\alpha^2\omega^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2\\
% \leq & \frac{60\omega^2\alpha^2}{1-15\omega^2} \sum_{t=0}^{T-1}\mathbb{E}\left\|\e_{t-1}\right\|^2 + 6\omega^2\alpha^2 \sigma^2 T + \frac{88\omega^2L^2\gamma^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\|\v_{t-1}\|^2  +6\omega^2\sum_{t=0}^{T-1}\mathbb{E}\left\|  \odelta_{t}\right\|^2\\
% & + \frac{18\omega^2L^2\gamma^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\|\v_{t-1} \right\|^2 + \frac{198\omega^2\alpha^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E}\left\| \e_{t-1}\right\|^2  + \frac{198\omega^2\alpha^2(\sigma^2 + \zeta^2)}{1-15\omega^2} + \frac{18\alpha^2\omega^2}{1-15\omega^2}\sum_{t=0}^{T-1}\mathbb{E} \left\|\odelta_{t}\right\|^2.
% \end{align*}
